Software Engineering for Fairness: A Case Study with Hyperparameter Optimization

We assert that it is the ethical duty of software engineers to strive to reduce software discrimination. This paper discusses how that might be done. This is an important topic since machine learning software is increasingly being used to make decisions that affect people's lives. Potentially, the application of that software will result in fairer decisions because (unlike humans) machine learning software is not biased. However, recent results show that the software within many data mining packages exhibits "group discrimination"; i.e. their decisions are inappropriately affected by "protected attributes"(e.g., race, gender, age, etc.). There has been much prior work on validating the fairness of machine-learning models (by recognizing when such software discrimination exists). But after detection, comes mitigation. What steps can ethical software engineers take to reduce discrimination in the software they produce? This paper shows that making \textit{fairness} as a goal during hyperparameter optimization can (a) preserve the predictive power of a model learned from a data miner while also (b) generates fairer results. To the best of our knowledge, this is the first application of hyperparameter optimization as a tool for software engineers to generate fairer software.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> section/background.tex <==
\section{Background and Motivation}
\label{background}

In this section, we will discuss the motivation and related work on Self Admitted Technical Debt. The term, Technical Debt was first introduced by Cunningham in 1993\cite{cunningham1993wycash}. But only recently we are observing a dire need to identify and resolve this issue. 

\subsection{Motivation}
Technical Debt is an unavoidable and necessary business reality in software industry. In 2012, after interviewing 35 software developer from different projects in different companies, both varying in size and type, Lim et al. concluded that developers are bound to leave TD while developing software products. That happens due to many factors such as increased workload or unrealistic deadline in projects, lack of knowledge, boredom or peer-pressure among developers, unawareness or short-term business goals of stakeholders, reuse of legacy or third party or open source code etc. Research also found that, stakeholders and project managers are mostly aware of such debt\cite{lim2012balancing}\cite{al2014explicating}. After observing five large scale projects, Wehaibi et al. found that, the amount of Technical Debt in a project is very low (only 3\% on average), yet they create significant amount of defects in the future and fixing such Technical Debts are more difficult than regular defects\cite{wehaibi2016examining}. Another study on five software large scale companies revealed that, TD contaminates other parts of a software system and most of the future interests are non-linear in nature with respect to time\cite{martini2015danger}. According to the SIG (Software Improvement Group) study of Nugroho et al., resolving TD has a Return On Investment (ROI) of 15\% in seven years\cite{nugroho2011empirical}. Guo et al. also found similar results and concluded that, the cost of resolving TD in future is twice as much as resolving immediately\cite{guo2011tracking}. Thus, software industry is getting more and more concerned for identifying and managing TD.


\subsection{Related Work}
Many research have been trying to identify TD as part of Code Smells using static code analysis\cite{marinescu2010incode}\cite{marinescu2004detection}\cite{marinescu2012assessing}\cite{zazworka2013case}\cite{fontana2012investigating}. But static code analysis have high rate of false alarms while imposing complex and heavy structures for identifying TD\cite{tsantalis2011identification}\cite{tsantalis2015assessing}\cite{graf2010speeding}\cite{ali2012application}. A more recent study showed that, TD can be identified using source code comments. In 2014, after studying four large scale open source software projects, Potdar and Shihab concluded that developers intentionally leave traces of TD in their comments. They defined such TD as Self Admitted Technical Debt\cite{potdar2014exploratory}. This particular type of TD are more visible yet light-weight than traditional static analysis approach and covers almost 3\% of the comments. Their study found 62 distinct keywords for identifying such TD. A similar work has been done by Faris et al.\cite{de2015contextualized} as well. In 2015, Maldonado et al. used five open source projects to manually classify different types of SATD \cite{maldonado2015detecting} and found that, SATD mostly contains Requirement Debt and Design Debt in source code comments. Their work is based on the 6 major classes of TD proposed by Alves et al.\cite{alves2014towards}. In 2017, Maldonado et al. successfully identified two types of SATD in 10 open source projects (average 63\% F1 Score) using Natural Language Processing (Max Entropy Stamford Classifier) using only 23\% training data\cite{maldonado2017using}. A different approach was introduced by Huang et al. in 2018. Using eight datasets, Huang build Naive Bayes Multinomial sub-classifier for each training dataset using Information Gain as Feature Selection. By implementing a boosting technique using all those sub-classifiers, they have found an average 73\% F1 scores for all datasets\cite{huang2018identifying}. According to our knowledge, this is the current state-of-the-art approach for identifying SATD in a project. A recent IDE for Ecliplse was also released using this technique for identifying SATD in java projects\cite{liu2018satd}.

A few study tried to understand the nature of SATD in the open source community. On an empirical study on five open source projects in Github, Maldonado et al. found that 75\% of the SATD gets removed, but the median lifetime of SATD ranges between 18-173 days\cite{maldonado2017empirical}. Another study tried to find the SATD introducing commits in Github using different features on change level\cite{yan2018automating}. Instead of using bag of word approach, a recent study also proposed word embedding as vectorization technique for identifying SATD\cite{flisar2018enhanced}. 

There is little consensus among developers and tools regarding the identification of TD. Also, different projects/teams consider different comments as TD\cite{zazworka2013case}\cite{kruchten2013technical}\cite{ernst2015measure}. Even though, TD, more specifically SATD can be identified somewhat fairly in a project using existing approach such as proposed by Huang et al.\cite{huang2018identifying}, such approach has a precision and recall of 75\% on average. Thus, a second look for verification is necessary for the developers and project managers before removing the TD with confidence. Such verification task is tedious and time-consuming. For such reasons, the software industry is still looking for a practical solution to identify Technical Debt\cite{yli2016software}. According to our knowledge, there is no work done to estimate the number of SATD in a project as well. In our work, we propose an estimation and verification technique that will reduce the cost of identifying and verifying SATD in a project by using a combination of AI and Human. This work will reduce the cost of verification while increasing the confidence of developers and/or project managers to identify SATD.

==> section/conclusion.tex <==
\section{Conclusion}
\label{conclusion}

One previous work named FARSEC identifies security related words and applies filters to remove not-security bug reports. FARSEC build prediction models with default configurations in learners from Weka. However, FARSEC does not achieve good prediction performance. In this work, we propose to apply hyperparameter optimization to learners and use a data balancing technique called SMOTE to oversample the imbalanced class in FARSEC datasets. Furthermore, we use a tuned version of SMOTE to address the imbalanced class isse. Our experiment results on FARSEC datasets shows that hyperparameer optimization can improve performance than default configuration. However, the improvement is limited and does not apply for all datasets. SMOTE and SMOTUNED can efficient improve the baseline prediction results.

==> section/design.tex <==
\section{Design}
\label{design}

\begin{figure}[t]
\centerline{\includegraphics[width=0.45\textwidth]{architecture.jpg}}
\caption{Framework for Hyperparameter Optimization in Security Bug Report Prediction.}    
\label{figure:framework}
\end{figure}

\subsection{Overview}
Figure~\ref{figure:framework} show the general framework of our proposed approaches. Basically, our work in this paper can be divided into two parts. On the one hand, we propose to use an optimizer called differential evolution (DE) to search for optimal configurations in different learners. On the other hand, we propose to leverage a novel oversampling technique called SMOTE to address the imbalanced class problem in bug report prediction. 

\subsection{Differential Evolution Optimizer}
In machine learning, an optimizer is usually working on a higher level of various learners to automatically tune learners' configurations. In simpler terms, optimizers shape the models into their most accurate possible forms in order to achieve optimal performance. There are a couple of optimizers that have been frequently used in software engineering area. In this paper, we choose a novel optimizer called differential evolution (DE) in tuning learners' hyperparameters.

% \textcolor{red}{why we use optimizer, because optimizers can greatly improve data miners}~\cite{agrawal2018better}, and \textcolor{red}{explain why we choose DE, FLASH and Tabu Search in our paper}.

When solving a global optimization problem, our natural requirement is to find an acceptable approximation of the global minimum point as quickly as possible. Differential evolution (DE)~\cite{storn1997differential} is one of the most popular heuristics for global optimization, and it has been successfully applied in various areas, where used as a method for parametric identification of complex models. In most scenarios, DE as a population-based method requires a very large number of fitness evaluations (which also means a large mount of computation time) in order to achieve an acceptable result. 

Basically, the differential evolution algorithm is a type of evolutionary algorithm~\cite{back1996evolutionary} in which the fittest individuals of a population are the ones that produce more offspring and therefore inherit the good traits of the parents. An iterative mutation algorithm where vector differences are used to create new candidate solutions. There are four steps in  differential evolution algorithm: \textit{initialization}, \textit{mutation}, \textit{crossover}, and \textit{selection}. 

\textbf{Initialization.} The first step is to create a population of individuals. An individual is an instantiating of the parameters of target function, in which works by generating random values for each parameter within the given bounds. This step also applies each individual of the population to the target function, and we keep the one with the best values after evaluation.

\textbf{Mutation.} For each individual in the population, we select three other individuals that are not the current one. We create a mutant individual by combining these three individuals, in which we compute the difference between two individuals and add that difference to the rest individual after multiplying a mutation factor to the difference. The mutation factor is a positive number usually less than 1.0 that controls the amplification difference between two individuals, and it is also used to avoid stagnation in the search process.

\textbf{Crossover.} The crossover process is to mix the information of the mutant with the information of the current individual to create a trail individual. This is done by changing the value at some position in the current individual with the ones in the mutant individual. For each position, we decide if the place to be replaced or not by crossover point. We generate the uniform random values between [0,1] and check if the values are less than the crossover point.

\textbf{Selection.} After generating our new trial vector, we need to denormalize it and evaluate it to measure how good it is by applying it to the target function. If this mutant is better than the current vector then we replace it with the new one. Otherwise, the trail individual is discarded. As a result, all the individuals of the next generation are as good as or better than their counterparts in the current generation.

All the above steps have to be repeated again for the remaining individuals, which completes the first iteration of the algorithm. After this process, some of the original vectors of the population will be replaced by better ones, and after many iterations, the whole population will eventually converge towards the optimal solution. Algorithm~\ref{algorithm:DE} shows the pseudocode of differential evolution algorithm.

\begin{algorithm}[t]
\small
\hspace{0.2cm}\begin{lstlisting}[xrightmargin=5.0ex,mathescape,frame=none,numbers=right]
def DE(np, cf, f):
  frontier = sets of guesses
  best = frontier.1 # any value at all
  lives = 1
  while (lives-->0):
    tmp = empty
    for i = 1 to |frontier|: # size of frontier
        old = frontier
        x,y,z = any three from frontier, picked at random
        new = copy(old)
        for j = 1 to |new|: # for all attributes
        if rand() < cf: # at probability cf
            new.j = x.j + f * (z.j - y.j) # ... change item j
        # end for
        new = new if better(new, old) else old
        tmp_i = new
        if better(new, best) then
            best = new
            lives++ # enable one more generation
        end
    # end for
    frontier = tmp
  # end while
  return best
  
\end{lstlisting}
\caption{Pseudocode of Differential Evolution}
\label{algorithm:DE}  
\end{algorithm}

\textbf{DE Parameters.} There are four parameters in differential algorithms, the mutation factor \textit{F}, crossover constant \textit{CR}, the size of population \textit{NP} and the number of iteration \textit{ITER}. Base on the previous advice from developers\footnote{http://cci.lbl.gov/cctbx\_sources/scitbx/differential\_evolution.py}, the following classical setting for the input can be considered. 1) Set the number of the population \textit{NP} to $10$ times the number of parameters. 2) Set mutation factor $\textit{F}=0.8$. Recent studies have found that selecting \textit{F} from the interval $[0.5, 1.0]$ randomly for each generation or for each difference vector improves convergence behaviour significantly, especially for noisy objective functions. 3) Set crossover constant $\textit{CR}=0.9$. It has also been found that setting \textit{CR} to a low value, e.g. $\textit{CR}=0.2$ helps optimizing separable functions since it fosters the search along the coordinate axes. On the contrary this choice is not effective if parameter dependence is encountered, something which is frequently occurring in real-world optimization problems rather than artificial test functions. So for parameter dependence the choice of $\textit{CR}=0.9$ is more appropriate. 4) Set the number of iteration \textit{ITER} to $3$, $10$, which are denoted as DE$3$ and DE$10$ respectively. A small number ($2$) is used to test the effects of a very CPU-light effort estimator. A larger number ($10$) is selected to check if anything is lost by restricting the inference to small iterations. Table~\ref{tbl:DEpara} lists all the DE parameters for different learners. 

% However, we need to keep in mind that different problems often require different settings for NP, F and CR. In our work, to make the parameter setting problem simple, we follow the suggested advice, i.e., set NP to 40 for tuning CART (we have 4 hyper-parameters to tune in CART) and 60 when tuning Random Forest (we have 6 hyper-parameters to tune in Random Forest). We also set F = 0.8 and CR = 0.9. In addition, the iteration is set to 100, which we believe is enough for us to achieve optimal solution, and can be comparable when we consider tuning time between parallel DE and our baseline, i.e., traditional sequential DE.

\begin{table}[!htbp]
\caption {List of parameters in DE algorithm for different learners.}
% \normalsize
\centering
\begin{tabular}{l|c|c|c|c}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{4}{c}{\cellcolor[HTML]{EFEFEF}\textbf{DE Parameter}} \\ \cline{2-5} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Learner}}} & \textbf{NP} & \textbf{F} & \textbf{CR} & \textbf{ITER} \\ \hline
Random Forest & 60 &  &  &  \\ \cline{1-2}
Logistic Regression & 30 &  &  &  \\ \cline{1-2}
Multilayer Perceptron & 60 &  &  &  \\ \cline{1-2}
K Nearest Neighbor & 20 &  &  &  \\ \cline{1-2}
Naive Bayes & 10 & \multirow{-5}{*}{0.8} & \multirow{-5}{*}{0.9} & \multirow{-5}{*}{3, 10} \\ \hline
\end{tabular}
\label{tbl:DEpara}
\end{table}


% \subsubsection{FLASH} FLASH~\cite{nair2017flash}~\cite{nair2018finding} is a sequential model-based method such as Bayesian optimization, is a useful strategy to find extremes of an unknown objective. FLASH is efficient because of its ability to incorporate prior belief as already measured solutions (or configurations), to help direct further sampling. Here, the prior represents the already known areas of the search (or performance optimization) problem. The prior can be used to estimate the rest of the points (or unevaluated configurations). Once one (or many) points are evaluated based on the prior, the posterior can be defined. The posterior captures the updated belief in the objective function. This step is performed by using a machine learning model, also called surrogate model. \textcolor{red}{to be continued...}


% \begin{algorithm}
% \small
% \hspace{0.2cm}\begin{lstlisting}[xrightmargin=5.0ex,mathescape,frame=none,numbers=right]
% def FLASH(uneval_configs, fitness, size, life):
%   # Add |size| number of randomly selected configurations to training data. 
%   # All the randomly selected configurations are measured
%   eval_configs = [measure(x) for x in sample(uneval_configs, size)]
%   # Remove the evaluations configuration from data
%   uneval_configs.remove(eval_configs)
%   # Till all the lives has been lost
%   while life > 0:
%     # build one CART model per objective
%     for o in objectives: model[o] = CART(eval_configs)
%     # Find and measure another point based on acquisition function
%     acquired_point = measure(acquisition_fn(uneval_configs, model))
%     eval_configs += acquired_point  # Add acquired point 
%     uneval_config -= acquired_point # Remove acquired point 
%     # Stopping Criteria
%     life -= 1
%   return best
  
% def acquisition_fn(uneval_configs, model, no_directions=10):  
%   # Predict the value of all the unevaluated configurations using model
%   predicted = model.predict(uneval_configs)
%   # If number of objectives is greater than 1 (In our setting len(objectives) = 2)
%   if len(objectives) > 1: # For multi-objective problems
%     return  Bazza( predicted )
%   else:  # For single-objective problems
%     return max(predicted)  
% \end{lstlisting}
% \caption{Pseudocode of FLASH}
% \label{fig:flash_frame}  
% \end{algorithm}

% \subsubsection{Tabu Search} Tabu Search using $\epsilon$-dominance, DART~\cite{fu2018building} is a meta-heuristic search method employing local search methods used for mathematical optimization. Tabu search uses a local or neighborhood search procedure to iteratively move from one potential solution x to an improved solution x' in the neighbourhood of x, until some stopping criterion has been satisfied~\cite{chen2018beyond}~\cite{du2013handbook}.  \textcolor{red}{to be continued...}




% \begin{table*}[!htb]
% \caption {Comparison of Hyperparameters of used learners in Weka and Scikit-learn.}
% \begin{tabular}{|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Learner}}} & \multicolumn{2}{c|}{\textbf{Hyperparameter}} \\ \cline{2-3} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textbf{Weka}} & \multicolumn{1}{c|}{\textbf{Scikit-learn}} \\ \hline
% Random Forest & \begin{tabular}[c]{@{}l@{}}bagSizePercent: 100\\ batchSize: 100\\ breakTiesRandomly: False\\ calcOutOfBag: False\\ computeAttributeImportance: False\\ debug: False\\ doNotCheckCapabilities: False\\ maxDepth: 0\\ numDecimaalPlaces: 2\\ numExecutionSlots: 1\\ numFeatures: 0\\ numIteration: 100\\ outputOutOfBagComplexityStatistics: Fasle\\ printClassifier: False\\ seed: 1\\ storeOutOfBagPredictions: False\end{tabular} &  \\ \hline
% Naive Bayes & \begin{tabular}[c]{@{}l@{}}batch size: 100\\ debug: False\\ displayModelInOldFormat: False\\ numDecimalPlaces: 2\\ useKernelEstimator: False\\ useSupervisedDiscretization: False\end{tabular} &  \\ \hline
% Logistic Regression & \begin{tabular}[c]{@{}l@{}}batchSize: 100\\ debug: False\\ doNotCheckCapabilities: False\\ maxIts: -1\\ numDecimalPlaces: 4\\ ridge: 1.0E-8\\ useConjugateGradientDescent: False\end{tabular} &  \\ \hline
% KNN & \begin{tabular}[c]{@{}l@{}}KNN: 1\\ batchSize: 100\\ crossValidate: False\\ debug: False\\ distanceWeighting: No distance weighting\\ doNotCheckCapabilities: False\\ meanSqured: False\\ nearestNeighbourSearchAlgorithm: LinearNNSearch\\ numDecimalPlaces: 2\\ windowSize: 0\end{tabular} &  \\ \hline
% Multilayer Perceptron & \begin{tabular}[c]{@{}l@{}}GUI: False\\ autoBuild: True\\ batchSize: 100\\ debug: False\\ decay: False\\ doNotCheckCapabilities: False\\ hiddenLayers: a\\ learningRate: 0.3\\ momentum: 0.2\\ nominalToBinaryFilter: True\\ normalizeAttributes: True\\ normalizeNumericClass: True\\ numDecimalPlaces: 2\\ reset: True\\ seed: 0\\ trainingTime: 500\\ validationSetSize: 0\\ validationThreshold: 20\end{tabular} &  \\ \hline
% \end{tabular}
% \end{table*}

\subsection{Data Balancing with SMOTE}



Imbalanced data typically refers to an issue with classification problems where the classes are not equally represented. For example, in a binary classification problem, the ratio of class $0$ and $1$ is $99:1$. There are many reasons why a dataset might be imbalanced, e.g., the data might simply be difficult to collect, or the category that we are targeting might be very rare in the population. A direct impact by imbalanced dataset is that the learned model will be biased. 

A number of methods are available to oversample a dataset used in a typical classification problem.
SMOTE~\cite{chawla2002smote} (Synthetic Minority Oversampling Technique), as a novel oversampling technique, works by creating synthetic samples based on the existing minority samples rather than replicating the minority samples. SMOTE takes the whole dataset as input, and increases the percentage of the minority class. As a result, the increasement of the instances available to each class makes the dataset more balanced. 

To be specific, SMOTE calculates the $k$ nearest neighbors for each minority class samples. Depending on the amount of oversampling required, one or more of the $k$-nearest neighbors are picked to create the synthetic samples. This amount is usually denoted by oversampling percentage (e.g., $50\%$ by default). The next step is to randomly create a synthetic sample along the line connecting two minority samples. This can be illustrated in Figure~\ref{figure:SMOTE} where the blue dots represent the minority class sample, and the red dots represent the synthetic samples.  

\begin{figure}[t]
\centerline{\includegraphics[width=0.4\textwidth]{SMOTE.jpg}}
\caption{An Illustration on How the SMOTE Technique Works.}    
\label{figure:SMOTE}
\end{figure}

Agrawal et al.~\cite{agrawal2018better} used an updated SMOTE in handling the data imbalanced problem in software defect prediction. In their work, the SMOTE algorithm can be broken down into two parts: (1) sub-sample the majority class (i.e., randomly delete some instances) and (2) super-sample the minority class (i.e., add synthetic instances). We applied a similar method in our work, and the detailed algorithm can be illustrated in Algorithm~\ref{algorithm:smote}.

\begin{algorithm}[t]
\small
\hspace{0.2cm}\begin{lstlisting}[xrightmargin=5.0ex,mathescape,frame=none,numbers=right]
def SMOTE(k=2, m=50%, r=2):
    while Majority > m do
        delete any majority item
    while Minority < m do
        add something_like(any minority item)
        
def something_like(X0):
    relevant = emptySet
    k1 = 0
    while(k1++ < 20) and size(found) < k {
        all = k1 nearest neighbours
        relevant += item in "all" of X0 class
    }
    Z = any of found
    Y = interpolate(X0, Z)
    return Y
    
def minkowski_distance(a, b, r):
    return ($\Sigma_{i}abs(a_{i}-b_{i})^{r})^{1/r}$

\end{lstlisting}
\caption{Pseudocode of SMOTE}
\label{algorithm:smote}  
\end{algorithm}

\begin{table}[!htbp]
\caption {SMOTE parameters and tuning range.}
\begin{tabular}{c|r|r|l}
\hline
\rowcolor[HTML]{EFEFEF}
\textbf{Para} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Defaults\\ Used by\\ SMOTE\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Tuning Range}} & \multicolumn{1}{c}{\textbf{Description}} \\ \hline
k & 5 & {[}1,20{]} & Number of neighbors. \\ \hline
m & 50\% & \begin{tabular}[c]{@{}r@{}}{[}50, 400{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number of synthetic examples\\ to create. Expressed as a \\percent of final training data.\end{tabular} \\ \hline
r & 2 & {[}1,6{]} & \begin{tabular}[c]{@{}l@{}}Power parameter for the\\ Minkowski distance metric.\end{tabular} \\ \hline
\end{tabular}
\label{tbl:SMOTEpara}
\end{table}

In addition, Agrawal et al.~\cite{agrawal2018better} also designed an auto-tuning version SMOTE named SMOTUNED that used different control parameters instead of the default parameters of SMOTE algorithm. Specifically, SMOTUNED uses differential evolution algorithm to explore the parameter space. As shown in Table~\ref{tbl:SMOTEpara}, the SMOTE algorithm has three parameters: 1) the number of neighbors $k$; 2) the percentage of synthetic examples created $m$; 3) the power of Minkowski distance metric $r$. 

In our work, we explore the usage of SMOTUNED in bug report prediction. We set the tuning ranges for each parameters in Table~\ref{tbl:SMOTEpara}. In order to reduce the noise by overpopulating the minority samples, we are not using $m$ as percentage but as the exact number of samples created. Note that since there are three parameters to optimize, as for differential evolution from Algorithm~\ref{algorithm:DE}, we set the number of population \textit{NP} to $30$, and use the same mutation factor \textit{F} and crossover constant \textit{CR} from Table~\ref{tbl:DEpara} and set the iteration \textit{ITER} to $10$.



==> section/discussion.tex <==
\section{Threats to Validity}
\label{threats}

As to any empirical study, biases can affect the final results. Therefore, conclusions drawn from this work must be considered with threats to validity in mind. In this section, we discuss the validity of our work.

\begin{enumerate}
    % \item \textbf{Sampling Validity.}
    \item \textbf{Learner Validity.} Lots of different machine learning algorithms have been developed to solve different classification problem tasks. An important note from David Wolpert is the ``No Free Lunch Theorems''. There is no one learner working for all problems. One reason for this is that each classification has its inherent biases. In this work, we do not explore the performance for different learners. To compare the work with FARSEC, we use the same learners as Peters did in their work.
    \item \textbf{Evaluation Validity.} On one hand, during our evaluation, we repeat our work 10 times and report the average performance results for different learners. On the other hand, we only set two versions of generations (i.e., 3 and 10) for learners and one version of generation (i.e., 10) for SMOTE in differential evolution algorithm. Larger number of generations could be further explored, but with more CPU efforts and time.
\end{enumerate}


==> section/evaluation.tex <==
\section{Evaluation and Results}
\label{evaluation}


% \begin{figure*}
%     \centering
%     \subfigure[train]{\includegraphics[width=0.24\textwidth]{figures/Chromium_train.png}}
%     \subfigure[farsecsq]{\includegraphics[width=0.24\textwidth]{figures/Chromium_farsecsq.png}}
%     \subfigure[farsectwo]{\includegraphics[width=0.24\textwidth]{figures/Chromium_farsectwo.png}}
%     \subfigure[farsec]{\includegraphics[width=0.24\textwidth]{figures/Chromium_farsec.png}}
%     \subfigure[clni]{\includegraphics[width=0.24\textwidth]{figures/Chromium_clni.png}}
%     \subfigure[clnifarsecsq]{\includegraphics[width=0.24\textwidth]{figures/Chromium_clnifarsecsq.png}}
%     \subfigure[clnifarsectwo]{\includegraphics[width=0.24\textwidth]{figures/Chromium_clnifarsectwo.png}}
%     \subfigure[clnifarsec]{\includegraphics[width=0.24\textwidth]{figures/Chromium_clnifarsec.png}}
%     \caption{Chromium datasets}
%     \label{fig:chromium}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \subfigure[train]{\includegraphics[width=0.24\textwidth]{figures/Wicket_train.png}} 
%     \subfigure[farsecsq]{\includegraphics[width=0.24\textwidth]{figures/Wicket_farsecsq.png}}
%     \subfigure[farsectwo]{\includegraphics[width=0.24\textwidth]{figures/Wicket_farsectwo.png}}
%     \subfigure[farsec]{\includegraphics[width=0.24\textwidth]{figures/Wicket_farsec.png}}
%     \subfigure[clni]{\includegraphics[width=0.24\textwidth]{figures/Wicket_clni.png}}
%     \subfigure[clnifarsecsq]{\includegraphics[width=0.24\textwidth]{figures/Wicket_clnifarsecsq.png}}
%     \subfigure[clnifarsectwo]{\includegraphics[width=0.24\textwidth]{figures/Wicket_clnifarsectwo.png}}
%     \subfigure[clnifarsec]{\includegraphics[width=0.24\textwidth]{figures/Wicket_clnifarsec.png}}
%     \caption{Wicket datasets}
%     \label{fig:wickt}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \subfigure[train]{\includegraphics[width=0.24\textwidth]{figures/Ambari_train.png}} 
%     \subfigure[farsecsq]{\includegraphics[width=0.24\textwidth]{figures/Ambari_farsecsq.png}}
%     \subfigure[farsectwo]{\includegraphics[width=0.24\textwidth]{figures/Ambari_farsectwo.png}}
%     \subfigure[farsec]{\includegraphics[width=0.24\textwidth]{figures/Ambari_farsec.png}}
%     \subfigure[clni]{\includegraphics[width=0.24\textwidth]{figures/Ambari_clni.png}}
%     \subfigure[clnifarsecsq]{\includegraphics[width=0.24\textwidth]{figures/Ambari_clnifarsecsq.png}}
%     \subfigure[clnifarsectwo]{\includegraphics[width=0.24\textwidth]{figures/Ambari_clnifarsectwo.png}}
%     \subfigure[clnifarsec]{\includegraphics[width=0.24\textwidth]{figures/Ambari_clnifarsec.png}}
%     \caption{Ambari datasets}
%     \label{fig:ambari}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \subfigure[train]{\includegraphics[width=0.24\textwidth]{figures/Camel_train.png}} 
%     \subfigure[farsecsq]{\includegraphics[width=0.24\textwidth]{figures/Camel_farsecsq.png}}
%     \subfigure[farsectwo]{\includegraphics[width=0.24\textwidth]{figures/Camel_farsectwo.png}}
%     \subfigure[farsec]{\includegraphics[width=0.24\textwidth]{figures/Camel_farsec.png}}
%     \subfigure[clni]{\includegraphics[width=0.24\textwidth]{figures/Camel_clni.png}}
%     \subfigure[clnifarsecsq]{\includegraphics[width=0.24\textwidth]{figures/Camel_clnifarsecsq.png}}
%     \subfigure[clnifarsectwo]{\includegraphics[width=0.24\textwidth]{figures/Camel_clnifarsectwo.png}}
%     \subfigure[clnifarsec]{\includegraphics[width=0.24\textwidth]{figures/Camel_clnifarsec.png}}
%     \caption{Camel datasets}
%     \label{fig:camel}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \subfigure[train]{\includegraphics[width=0.24\textwidth]{figures/Derby_train.png}} 
%     \subfigure[farsecsq]{\includegraphics[width=0.24\textwidth]{figures/Derby_farsecsq.png}}
%     \subfigure[farsectwo]{\includegraphics[width=0.24\textwidth]{figures/Derby_farsectwo.png}}
%     \subfigure[farsec]{\includegraphics[width=0.24\textwidth]{figures/Derby_farsec.png}}
%     \subfigure[clni]{\includegraphics[width=0.24\textwidth]{figures/Derby_clni.png}}
%     \subfigure[clnifarsecsq]{\includegraphics[width=0.24\textwidth]{figures/Derby_clnifarsecsq.png}}
%     \subfigure[clnifarsectwo]{\includegraphics[width=0.24\textwidth]{figures/Derby_clnifarsectwo.png}}
%     \subfigure[clnifarsec]{\includegraphics[width=0.24\textwidth]{figures/Derby_clnifarsec.png}}
%     \caption{Derby datasets}
%     \label{fig:derby}
% \end{figure*}



% \begin{table}[!htbp]
% \caption {Recall result from FARSEC, default Scikit-learn and DE tuning with Scikit-learn.}
% \small
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|c|r|c|r|c|r}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Weka\\ (FARSEC)\end{tabular}} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}Scikit-learn} & \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Scikit-learn\\ DE Tuning\end{tabular}} \\ \cline{3-8} 
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Project}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Filter}} & Learner & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}pd} & Learner & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}pd} & Learner & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}pd} \\ \hline
%  & train & LR & 15.7 & MP & 15.7 & NB & \textbf{49.6} \\ 
%  & farsecsq & RF & 14.8 & RF & 37.4 & NB & \textbf{72.2} \\  
%  & farsectwo & LR & 15.7 & MP & 15.7 & NB & \textbf{33.0} \\  
%  & farsec & LR & 15.7 & MP & 15.7 & NB & \textbf{45.2} \\ 
%  & clni & LR & 15.7 & MP & 15.7 & NB & \textbf{34.8} \\
%  & clnifarsecsq & MP & 49.6 & MP & 57.4 & MP & \textbf{66.1} \\ 
%  & clnifarsectwo & LR & 15.7 & MP & 15.7 & NB & \textbf{50.4} \\ 
% \multirow{-8}{*}{Chromium} & clnifarsec & LR & 15.7 & MP & 15.7 & NB & \textbf{45.2} \\ \hline
%  & train & NB & 16.7 & NB & 0 & NB & 0 \\ 
%  & farsecsq & LR & 66.7 & NB & 83.3 & NB & 83.3 \\ 
%  & farsectwo & LR & 66.7 & NB & 66.7 & NB & 50 \\ 
%  & farsec & LR & 33.3 & NB & 66.7 & NB & 66.7 \\ 
%  & clni & NB & 0 & NB & 0 & MP & \textbf{16.7} \\ 
%  & clnifarsecsq & LR & 33.3 & NB & 83.3 & NB & 50 \\
%  & clnifarsectwo & LR & 33.3 & NB & 66.7 & NB & 50 \\ 
% \multirow{-8}{*}{Wicket} & clnifarsec & LR & 50 & MP & 66.7 & NB & 66.7 \\ \hline
%  & train & MP & 14.3 & LR & 28.6 & LR & 28.6 \\ 
%  & farsecsq & RF & 42.9 & RF & 42.9 & RF & \textbf{57.1} \\
%  & farsectwo & RF & 57.1 & RF & 42.8 & RF & \textbf{57.1} \\
%  & farsec & MP & 14.3 & MP & 28.6 & RF & \textbf{57.1} \\  
%  & clni & MP & 14.3 & LR & 28.6 & LR & 28.6 \\ 
%  & clnifarsecsq & RF & 57.1 & RF & 57.1 & RF & 57.1 \\ 
%  & clnifarsectwo & RF & 28.6 & RF & 42.9 & RF & \textbf{57.1} \\ 
% \multirow{-8}{*}{Ambari} & clnifarsec & RF & 14.3 & LR & 28.5 & RF & \textbf{57.1} \\ \hline
%  & train & LR & 11.1 & NB & 16.7 & MP & 16.7 \\ 
%  & farsecsq & RF & 16.7 & RF & 38.9 & RF & \textbf{44.4} \\ 
%  & farsectwo & LR & 50 & NB & 61.1 & RF & 44.4 \\ 
%  & farsec & LR & 16.7 & NB & 22.2 & NB & 22.2 \\  
%  & clni & NB & 16.7 & NB & 16.7 & NB & 16.7 \\  
%  & clnifarsecsq & MP & 16.7 & RF & 27.8 & RF & \textbf{44.4} \\  
%  & clnifarsectwo & MP & 11.1 & NB & 61.1 & NB & 61.1 \\ 
% \multirow{-8}{*}{Camel} & clnifarsec & LR & 16.7 & NB & 22.2 & NB & 22.2 \\ \hline
%  & train & NB & 38.1 & NB & 45.2 & NB & 45.2 \\ 
%  & farsecsq & KNN & 54.8 & KNN & 35.7 & KNN & \textbf{59.5} \\ 
%  & farsectwo & RF & 47.6 & RF & 42.9 & LR & \textbf{59.5} \\ 
%  & farsec & NB & 38.1 & NB & 47.6 & NB & 47.6 \\ 
%  & clni & RF & 23.8 & NB & 45.2 & NB & 45.2 \\ 
%  & clnifarsecsq & KNN & 54.8 & RF & 71.4 & KNN & 59.5 \\ 
%  & clnifarsectwo & RF & 35.7 & RF & 35.7 & LR & \textbf{59.5} \\ 
% \multirow{-8}{*}{Derby} & clnifarsec & NB & 38.1 & NB & 47.6 & NB & 47.6 \\ \hline
% \end{tabular}
% }
% \label{tbl:tuningRecall}
% \end{table}


\begin{table*}[!htbp]
\caption {Recall and false positive results from FARSEC, default Scikit-learn and DE tuning with Scikit-learn., SMOTE with Scikit-learn and SMOTUNED with Scikit-learn.}
% \small
\centering
% \begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|l|c|r|r|c|r|r|c|r|r|c|r|r}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Weka\\ (FARSEC)\end{tabular}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Scikit-learn\\ DE Tuning\end{tabular}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Scikit-learn\\ SMOTE\end{tabular}}} & \multicolumn{3}{c}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}c@{}}Scikit-learn\\ SMOTUNED\end{tabular}}} \\ \cline{3-14} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Project}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Filter}}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} \\ \hline
 & train & LR & 15.7 & 0.2 & NB & 46.9 & 6.8 & NB & 68.7 & 24.1 & \cellcolor[HTML]{EFEFEF}MP & \cellcolor[HTML]{EFEFEF}73.9 & 17.8 \\  
 & farsecsq & RF & 14.8 & 0.3 & LR & 64.3 & 10.3 & NB & 80.0 & 31.5 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}84.3 & 25.1 \\  
 & farsectwo & LR & 15.7 & 0.2 & NB & 40.9 & 6.5 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}78.3 & 27.6 & RF & 77.4 & 23.1 \\  
 & farsec & LR & 15.7 & 0.2 & NB & 46.1 & 6.9 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}80.8 & 36.1 & MP & 72.2 & 14.9 \\  
 & clni & LR & 15.7 & 0.2 & NB & 30.4 & 4.1 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}74.8 & 24.8 & MP & 72.2 & 13.6 \\  
 & clnifarsecsq & MP & 49.6 & 3.8 & MP & 72.2 & 14.2 & NB & 82.6 & 30.4 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}86.1 & \cellcolor[HTML]{EFEFEF}25.6 \\  
 & clnifarsectwo & LR & 15.7 & 0.2 & NB & 50.4 & 7.0 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}79.1 & \cellcolor[HTML]{EFEFEF}29.9 & MP & 74.8 & 12.8 \\  
\multirow{-8}{*}{Chromium} & clnifarsec & LR & 15.7 & 0.2 & NB & 47.8 & 10.4 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}78.3 & \cellcolor[HTML]{EFEFEF}29 & MP & 74.7 & 17.1 \\ \hline
 & train & NB & 16.7 & 7.1 & NB & 0.0 & 5.1 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 32 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 12.1 \\  
 & farsecsq & LR & 66.7 & 38.3 & NB & 50.0 & 44.5 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}83.3 & 71.3 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}83.3 & 66.8 \\  
 & farsectwo & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}66.7 & 36.6 & NB & 50.0 & 42.3 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 68.2 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 62.9 \\  
 & farsec & LR & 33.3 & 8.1 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 23.1 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 43.9 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 26.1 \\  
 & clni & NB & 0.0 & 5.5 & MP & 16.7 & 2.4 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}50.0 & 21.1 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}50.0 & 12.5 \\  
 & clnifarsecsq & LR & 33.3 & 25.5 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}83.3 & 66.8 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}83.3 & 66.8 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}83.3 & 66.8 \\  
 & clnifarsectwo & LR & 33.3 & 27.7 & NB & 50.0 & 39.9 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 61.3 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 61.3 \\  
\multirow{-8}{*}{Wicket} & clnifarsec & LR & 50.0 & 10.5 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 23.1 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 38.9 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & 22.9 \\ \hline
 & train & MP & 14.3 & 1.6 & LR & 28.6 & 0.8 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}57.1 & 20.1 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 10.8 \\  
 & farsecsq & RF & 42.9 & 14.4 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 2.8 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}57.1 & 30.4 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 17.2 \\  
 & farsectwo & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 3.0 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 2.8 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 22.1 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 17.8 \\  
 & farsec & MP & 14.3 & 4.9 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 2.0 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}57.1 & 19.9 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}57.1 & 7.1 \\  
 & clni & MP & 14.3 & 2.6 & LR & 28.6 & 0.8 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}57.1 & 12.4 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}57.1 & 8.9 \\  
 & clnifarsecsq & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 7.7 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 2.4 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 13.4 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 7.1 \\  
 & clnifarsectwo & RF & 28.6 & 4.5 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 2.8 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 13.0 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 5.1 \\  
\multirow{-8}{*}{Ambari} & clnifarsec & RF & 14.3 & 0.0 & RF & 57.1 & 2.4 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & 7.9 & RF & 57.1 & 3.9 \\ \hline
 & train & LR & 11.1 & 3.5 & MP & 16.7 & 1.5 & NB & 33.3 & 27.4 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}44.4 & 35.9 \\  
 & farsecsq & RF & 16.7 & 11.4 & RF & 44.4 & 24.7 & RF & 44.4 & 20.5 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}55.6 & 23.4 \\  
 & farsectwo & LR & 50.0 & 41.8 & RF & 44.4 & 17.6 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}61.1 & 71.0 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}61.1 & 53.1 \\  
 & farsec & LR & 16.7 & 6.9 & NB & 22.2 & 12.4 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}33.3 & 39.4 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}33.3 & 28.0 \\  
 & clni & NB & 16.7 & 12.3 & NB & 16.7 & 7.9 & NB & 33.3 & 33.6 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}38.9 & 35.3 \\  
 & clnifarsecsq & MP & 16.7 & 13.9 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}38.9 & 14.9 & RF & 27.8 & 12.4 & RF & 33.3 & 15.6 \\  
 & clnifarsectwo & MP & 11.1 & 7.7 & NB & 61.1 & 50.0 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}72.2 & 64.9 & NB & 61.1 & 51.9 \\  
\multirow{-8}{*}{Camel} & clnifarsec & LR & 16.7 & 5.0 & NB & 22.2 & 11.6 & LR & 33.3 & 24.9 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}38.9 & 34.4 \\ \hline
 & train & NB & 38.1 & 6.8 & NB & 47.6 & 39.3 & NB & 54.7 & 22.2 & \cellcolor[HTML]{EFEFEF}MP & \cellcolor[HTML]{EFEFEF}59.5 & 20.7 \\  
 & farsecsq & KNN & 54.8 & 29.9 & KNN & 59.5 & 40.6 & RF & 54.7 & 51.7 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}66.7 & 51.5 \\  
 & farsectwo & RF & 47.6 & 12.4 & LR & 59.5 & 24.2 & RF & 47.6 & 27.9 & \cellcolor[HTML]{EFEFEF}MP & \cellcolor[HTML]{EFEFEF}66.7 & 33.6 \\  
 & farsec & NB & 38.1 & 6.3 & NB & 47.6 & 4.1 & NB & 57.1 & 21.0 & \cellcolor[HTML]{EFEFEF}MP & \cellcolor[HTML]{EFEFEF}59.5 & 19.0 \\  
 & clni & RF & 23.8 & 0.4 & NB & 45.2 & 3.5 & NB & 57.7 & 16.8 & \cellcolor[HTML]{EFEFEF}MP & \cellcolor[HTML]{EFEFEF}61.9 & 24.5 \\  
 & clnifarsecsq & KNN & 54.8 & 29.9 & KNN & 59.5 & 42.4 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}76.2 & 74.7 & RF & 69.0 & 65.1 \\  
 & clnifarsectwo & RF & 35.7 & 9.2 & LR & 59.5 & 24.2 & RF & 54.8 & 36.5 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}61.9 & 30.3 \\  
\multirow{-8}{*}{Derby} & clnifarsec & NB & 38.1 & 6.8 & NB & 47.6 & 3.9 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}61.9 & 28.8 & NB & 57.1 & 10.9 \\ \hline
\end{tabular}
% \end{adjustbox}
\label{tbl:tuningRecall}
\end{table*}

\begin{figure*}[!t]
\centering
\scriptsize
\begin{tabular}{cc}
  
  % BEGIN SECOND IMG
  \begin{tikzpicture}
	\begin{axis}[
		height=4cm,
		width=8cm,
		ymax=70,
		%grid=major,
		xlabel={All values (sorted)},
        ylabel={Change in $pd$}
	]
	\addplot table [x=a, y=DE, col sep=comma, mark=none] {detla_pd.csv};
	%\addlegendentry{DE}
    \addplot table [x=a, y=SMOTE, col sep=comma,mark=none] {detla_pd.csv};
	%\addlegendentry{SMOTE}
	\addplot table [x=a, y=SMOTETUNE, col sep=comma,mark=none] {detla_pd.csv};
	%\addlegendentry{SMOTUNED}
	\end{axis}
    \end{tikzpicture} 
  % END SECOND IMG
  & 
  % BEGIN FIRST IMG
 \begin{tikzpicture}
	\begin{axis}[
		height=4cm,
		width=8cm,
		ymax=70,
		%grid=major,
		xlabel={All values (sorted)},
        ylabel={Change in $pf$},   
        legend style={at={(0.25,0.95)},anchor=north} 
	]
	\addplot table [x=a, y=DE, col sep=comma, mark=none] {detla_pf.csv};
	\addlegendentry{DE}
    \addplot table [x=a, y=SMOTE, col sep=comma,mark=none] {detla_pf.csv};
	\addlegendentry{SMOTE}
	\addplot table [x=a, y=SMOTETUNE, col sep=comma,mark=none] {detla_pf.csv};
	\addlegendentry{SMOTETUNE}
%  	\legend{};
	\end{axis}
    \end{tikzpicture}
  % END FIRST IMG
  
  \\~\\
  % BEGIN THIRD IMG
  \begin{tikzpicture}
	\begin{axis}[
		height=4cm,
		width=8cm,
		ymax=90,
		%grid=major,
		xlabel={All values (sorted)},
        ylabel={$pd$},
        legend columns=-1
	]
	\addplot table [x=id, y=weka_pd, col sep=comma, mark=none] {sec2.csv};
	\addlegendentry{WEKA}
    \addplot table [x=id, y=st_pd, col sep=comma,mark=none] {sec2.csv};
	\addlegendentry{SMOTUNED}
	\legend{};
	\end{axis}
    \end{tikzpicture} 
  % END THIRD IMG
  &
  % BEGIN FORTH IMG
  \begin{tikzpicture}
	\begin{axis}[
		height=4cm,
		width=8cm,
		ymax=90,
		%grid=major,
		xlabel={All values (sorted)},
        ylabel={$pf$},
        legend columns=-1,
        legend style={at={(0.35,0.95)},anchor=north}
	]
	\addplot table [x=id, y=weka_pf, col sep=comma, mark=none, name path=A] {sec2.csv};
	\addlegendentry{WEKA}
    \addplot table [x=id, y=st_pf, col sep=comma,mark=none, name path=B] {sec2.csv};
	\addlegendentry{SMOTUNED}
	\end{axis}
    \end{tikzpicture} 
  % END FORTH IMG
\end{tabular}
\caption{A comparison of changes in pd and pf values among DE, SMOTE and SMOTUNED, and a comparison of pd and pf values between WEKA and SMOTUNED}
\end{figure*}

We now answer the following research questions:

\begin{tcolorbox}[enhanced,width=3.4in,size=fbox,
    fontupper=\normalsize\bfseries,drop shadow southwest,sharp corners]
(RQ1.) Can hyperparameter optimization technique improves prediction performance than using the ``off-the-shelf'' default configurations in learners for all datasets?
\end{tcolorbox}

As we discussed above, FARSEC uses default hyperparameter setting of different learners in Weka when performing prediction. Since we implement default prediction learners and apply hyperparameter tuning in scikit-learn, we firstly compare the prediction results from two different implementations over the same datasets. 

In our experiment, we describe a filter to a project as a dataset. We use 10-fold cross validation for each learner during the training phase, and we compute the median result of g-measure from 10 repetitive experiments. Cross validation provides a good projection of expected error of a model built on the full dataset. The learner with the highest computed g-measure is selected as candidate learner. We then rebuild the model with the candidate learner with the whole training dataset, and experiment on the separate testing dataset. 

These figures present performance results from candidate learners on all 40 datasets. However, we have no idea what is the selection methodology from FARSEC when its performance results are reported for each dataset. From these results we can see, scikit-learn achieves a similar performance (e.g., recall) to Weka on  most of 40 datasets.

We further investigate whether hyperparameter optimization improves prediction performance. In our experiment, as we discussed before, we only target on achieving a high g-measure performance measure. In general, a higher g-measure can be achieved by three ways:

\begin{itemize}
    \item A higher recall and a lower false positive rate
    \item A lower or the same recall and a lower false positive rate
    \item A higher recall and a higher or the same false positive rate
\end{itemize}

Therefore, a higher g-measure might be a trade-off between recall and false positive rate. We collect the performance results of the rest measures when getting the target measure result. Especially, for imbalanced datasets, we care more about the recall measure, for which we are pursuing high false positive with low false negative. Table~\ref{tbl:tuningRecall} takes a close look at the hyperparameter optimization result of the recall. We highlight the highest recall value with shadow among all approaches. Hyperparameter optimization improves the recall on 18 datasets and only only 7 of which are among the best results. This would indicate that the benefit of using hyperparameter optimization is limited.

To sum up, for this research question, we can conclude that hyperparameter tuning  improves prediction performance than using the ``off-the-shelf'' default configurations in learners. However, it does not apply to all the datasets.




\begin{tcolorbox}[enhanced,width=3.4in,size=fbox,
    fontupper=\normalsize\bfseries,drop shadow southwest,sharp corners]
(RQ2.) Can oversampling techniques like SMOTE and tuned SMOTE address the imbalanced class problem in dataset?
\end{tcolorbox}

Table~\ref{tbl:tuningRecall} also show the prediction results of SMOTE with default parameters and tuned parameters. From these results, especially from Table~\ref{tbl:tuningRecall} we can observe that, the SMOTE-based oversampling approaches bring great improvements on the recall metrics, most of which are among the highest values of all compared approaches. The tuned version of SMOTE achieve the same results with regard to recall on the Wicket and Ambari datasets and improves better on the Camel and Derby datasets. Chromium dataset is a litter different case, in which SMOTE achieves higher recall on 5 out of 8 datasets than SMOTUNED. However, as we discuss before, SMOTUNED aims to achieves a higher g-measure, and in this case, a lower false positive rate is achieved at the cost of a lower recall results.



\begin{table*}[!htbp]
\centering
\caption{Average runtime (in minute) of tuning different learners' hyperparameters and SMOTE's hyperparameters.}
\begin{tabular}{c|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
\hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DE3}} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DE10}} & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{SMOTUNED}} \\ \cline{2-16} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Project}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{NB}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{RF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{MP}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{LR}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{KNN}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{NB}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{RF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{MP}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{LR}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{KNN}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{NB}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{RF}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{MP}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{LR}} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{KNN}} \\ \hline
Chromium & \textless{}1 & 14 & 288 & \textless{}1 & 151 & \textless{}1 & 39 & 435 & 4 & 398 & \textless{}1 & \textless{}1 & 6 & \textless{}1 & 11 \\
Wicket & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 & \textless{}1 & 2 & 6 & \textless{}1 & \textless{}1 & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 \\ 
Ambari & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 & \textless{}1 & 2 & 6 & \textless{}1 & \textless{}1 & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 \\ 
Camel & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 & \textless{}1 & 2 & 6 & \textless{}1 & \textless{}1 & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 \\
Derby & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 & \textless{}1 & 2 & 6 & \textless{}1 & \textless{}1 & \textless{}1 & \textless{}1 & 4 & \textless{}1 & \textless{}1 \\ \hline
\end{tabular}
\label{tbl:tuningtime}
\end{table*}

We also could notice that the best learner with SMOTE and SMOTUNED for each dataset alters when compared with FARSEC and default implementation with Scikit-learn. This might indicate that ``better data'' could be better than ``better data miners'', which means data preprocessing could be more efficient than switching to another data miners on some datasets.

For this research question, we answer ``yes'' since the performance increment seen above is much better than default learners and even the tuned learners.

\begin{tcolorbox}[enhanced,width=3.4in,size=fbox,
    fontupper=\normalsize\bfseries,drop shadow southwest,sharp corners]
(RQ3.) Is the cost of running hyperparameter optimization, tuned SMOTE worth the performance improvement in terms of runtimes?
\end{tcolorbox}

As we discussed in Section~\ref{design}, the search space of hyperparameters, i.e., the number of population, is set to 10 times of the number of hyperparameters. We use two different iterations, i.e., 3 and 10, in the hyperparameter tuning process and iteration number of 10 in SMOTUNED. Table~\ref{tbl:tuningtime} shows the average runtime of hyperparameter optimization and SMOTUNED. Looking over this table, there are two factors that influence the runtime: the size of dataset and the type of learner. Small datasets such as Wicket, Ambari, Camel and Derby have about 500 entries of data. In general, the tuning process is not slow, which takes less than 10 minutes for all learners. However, for large dataset like Chromium which has about 20,000 entries of data, except for multilayer perceptron and KNN, the tuning time for the rest learners in all cases are also acceptable.

Hence, we answer this RQ as ``yes'', the cost of tuning data mining learners and SMOTE is not high and worth the performance improvement.



==> section/experiment.tex <==
\section{Experiment}
\label{experiment}

\subsection{Bug Report Datasets}

Datasets used in our experiment are the same as Peters used in FARSEC, in which historical bugs reports from five projects are chosen: four from Ohira et al. (i.e., Wicket\footnote{https://wicket.apache.org/}, Ambari\footnote{http://ambari.apache.org/}, Camel\footnote{http://camel.apache.org/}, Derby\footnote{http://db.apache.org/derby/})~\cite{ohira2015dataset}, and a subset of bug reports from the Chromium project\footnote{https://www.chromium.org/Home}. FARSEC preprocessed the raw datasets with several steps, i.e., tokenize text, remove stop words and unwanted terms, calculate tf-idf (term frequency-inverse document frequency) values and construct term-document frequency matrix.

\begin{table}[!htbp]
\caption {Different Filters used in FARSEC.}
\centering
\begin{tabular}{l|l}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Filter}} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Description}} \\ \hline
farsecsq & \begin{tabular}[c]{@{}l@{}}Apply the Jalali et al.~\cite{jalali2008optimizing} support function\\ to the frequency of words found in SBRs\end{tabular} \\ \hline
farsectwo & \begin{tabular}[c]{@{}l@{}}Apply the Graham version~\cite{graham2004hackers} of multiplying \\ the frequency by two.\end{tabular} \\ \hline
farsec & Apply no support function. \\ \hline
clni & Apply CLNI filter to non-filtered data. \\ \hline
clnifarsec & Apply CLNI filter to farsec filtered data. \\ \hline
clnifarsecsq & Apply CLNI filter to farsecsq filtered data. \\ \hline
clnifarsectwo & Apply CLNI filter to farsectwo filtered data. \\ \hline
\end{tabular}
\label{tbl:farsecFilter}
\end{table}

FARSEC also applied multiple filters to remove NSBRs with security related keywords. Table~\ref{tbl:farsecFilter} lists all the filters used in FARSEC. FARSEC filtering method is mainly based on Graham's Bayesian filter~\cite{graham2004hackers}. For example, FARSEC used support functions to the frequency of the words found in SBRs to reduce mislabelled SBRs. In addition, FARSEC applied an noise detection algorithm called CLNI (Closet List Noise Identification)~\cite{kim2011dealing} method to deal with noise in prediction. A threshold score (e.g., $0.75$) is set to remove any NSBRs above the score.

All the training datasets are separated from the testing dataset in FARSEC. Each training dataset applied one specific filter, while a training dataset named ``train'' does not apply any filter. Table~\ref{tbl:farsecDataset} shows the charactersitics of the FARSEC datasets. As we can see from the table, the major challenge we face with these datasets is the imbalanced class problem, i.e., the number of SBRs occupies a small portion of the datasets.

\begin{table}[!htbp]
\caption {Imbalanced characteristics of bug report datasets from FARSEC.}
\small
\centering
\begin{tabular}{c|l|c|r|r}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Project} & \multicolumn{1}{c|}{\textbf{Filter}} & \textbf{\#SBR} & \multicolumn{1}{c|}{\textbf{\#BR}} & \multicolumn{1}{c}{\textbf{SBRs(\%)}} \\ \hline
\multirow{8}{*}{Chromium} & train & \multirow{8}{*}{77} & 20970 & 0.4 \\  
 & farsecsq &  & 14219 & 0.5 \\ 
 & farsectwo &  & 20968 & 0.4 \\  
 & farsec &  & 20969 & 0.4 \\  
 & clni &  & 20154 & 0.4 \\  
 & clnifarsecsq &  & 13705 & 0.6 \\  
 & clnifarsectwo &  & 20152 & 0.4 \\  
 & clnifarsec &  & 20153 & 0.4 \\ \hline
\multirow{8}{*}{Wicket} & train & \multirow{8}{*}{4} & 500 & 0.8 \\
 & farsecsq &  & 136 & 2.9 \\  
 & farsectwo &  & 143 & 2.8 \\  
 & farsec &  & 302 & 1.3 \\  
 & clni &  & 392 & 1.0 \\  
 & clnifarsecsq &  & 46 & 8.7 \\  
 & clnifarsectwo &  & 49 & 8.2 \\  
 & clnifarsec &  & 196 & 2.0 \\ \hline
\multirow{8}{*}{Ambari} & train & \multirow{8}{*}{22} & 500 & 4.4 \\  
 & farsecsq &  & 149 & 14.8 \\  
 & farsectwo &  & 260 & 8.5 \\  
 & farsec &  & 462 & 4.8 \\  
 & clni &  & 409 & 5.4 \\  
 & clnifarsecsq &  & 76 & 28.9 \\ 
 & clnifarsectwo &  & 181 & 12.2 \\  
 & clnifarsec &  & 376 & 5.9 \\ \hline
\multirow{8}{*}{Camel} & train & \multirow{8}{*}{14} & 500 & 2.8 \\  
 & farsecsq &  & 116 & 12.1 \\ 
 & farsectwo &  & 203 & 6.9 \\  
 & farsec &  & 470 & 3.0 \\  
 & clni &  & 440 & 3.2 \\  
 & clnifarsecsq &  & 71 & 19.7 \\  
 & clnifarsectwo &  & 151 & 9.3 \\  
 & clnifarsec &  & 410 & 3.4 \\ \hline
\multirow{8}{*}{Derby} & train & \multirow{8}{*}{46} & 500 & 9.2 \\  
 & farsecsq &  & 57 & 80.7 \\  
 & farsectwo &  & 185 & 24.9 \\  
 & farsec &  & 489 & 9.4 \\  
 & clni &  & 446 & 10.3 \\  
 & clnifarsecsq &  & 48 & 95.8 \\  
 & clnifarsectwo &  & 168 & 27.4 \\  
 & clnifarsec &  & 435 & 10.6 \\ \hline
\end{tabular}
\label{tbl:farsecDataset}
\end{table}


\subsection{Evaluation Metrics}

For the performance of the prediction models, we use TP, TN, FP and FN to denote True Positive, True Negative, False Positive and False Negative respectively. These metrics make up the confusion matrix, which is a breakdown of predictions into a table showing correct predictions and incorrect predictions. We also report the probability of detection \textit{pd} (i.e., recall), probability of false alarm \textit{pf} (i.e., false positive rate), precision, f-measure (i.e., f1-score) and g-measure. 

% Different metrics are chosen according to different cases. 

% \noindent
% \renewcommand\arraystretch{1.5}
% \setlength\tabcolsep{0pt}
% \begin{table}[t]
% \caption {Confusion matrix.}
% \centering
% \begin{tabular}{c >{\bfseries}r @{\hspace{0.7em}}c @{\hspace{0.4em}}c @{\hspace{0.7em}}l}
%   \multirow{10}{*}{\rotatebox{90}{\parbox{1.1cm}{\bfseries\centering actual\\ value}}} & 
%     & \multicolumn{2}{c}{\bfseries Prediction outcome} & \\
%   & & \bfseries $1$ & \bfseries $0$ & \bfseries Total \\
%   & $1$ & \MyBox{True}{Positive} & \MyBox{False}{Negative} & TP+FN \\[2.4em]
%   & $0$ & \MyBox{False}{Positive} & \MyBox{True}{Negative} & FP+FN \\ \\
%   & Total & TP+FP & FN+TN &
% \end{tabular}
% \label{tbl:cmatrix}
% \end{table}


\begin{eqnarray}
    \mathit{pd} &=& \frac{\mathit{TP}}{\mathit{TP}+\mathit{FN}} \\
    \mathit{pf} &=& \frac{\mathit{FP}}{\mathit{FP}+\mathit{TN}} \\
    \mathit{prec} &=& \frac{\mathit{TP}}{\mathit{TP}+\mathit{FP}} \\
    \mathit{f\textnormal{-}measure} &=& \frac{2 \times \mathit{pd} \times \mathit{prec}}{\mathit{pd}+\mathit{prec}} \\
    \mathit{g\textnormal{-}measure} &=& \frac{2 \times \mathit{pd} \times (1-\mathit{pf})}{\mathit{pd} + (1-\mathit{pf})}
\end{eqnarray}

Among these evaluation metrics, recall is a measure of classifier's completeness while precision is a measure of classifier's exactness. F-measure, as a harmonic average of precision and recall, seeks for  balanced between them. A good predictor is expected to achieve a high recall along with a low false positive rate precision. Base on this insight, we choose to achieve a high G-measure as our target in hyperparameter tuning, especially when there is an uneven class distribution.

% Note that we we do not choose recall as an evaluation metric, because in some cases a high recall also comes with a high false-positive rate.

% Note that F-measure is usually used to seek . Therefore, F-measure might be a good measure when there is an uneven class distribution (large number of Actual Negatives). \textcolor{red}{that's why we choose to tune F-score}


% \begin{table}
% % \large
% \caption {A list of evaluation metrics.}
% \label{table:metrics} 
% \begin{tabular}{|c|c|l|l|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{\textbf{Actual}} \\ \cline{3-4} 
% \multicolumn{2}{|c|}{} & yes & no \\ \hline
% \multirow{2}{*}{\textbf{Predicted}} & yes & TP & FP \\ \cline{2-4} 
%  & no & FN & TN \\ \hline
% \multirow{2}{*}{\textbf{Recall}} & \multicolumn{3}{c|}{\multirow{2}{*}{$\frac{TP}{TP+FN}$}} \\
%  & \multicolumn{3}{c|}{} \\ 
% \multirow{2}{*}{\textbf{Precision}} & \multicolumn{3}{c|}{\multirow{2}{*}{$\frac{TP}{TP+FP}$}} \\
%  & \multicolumn{3}{c|}{} \\ 
% \multirow{2}{*}{\textbf{F-measure}} & \multicolumn{3}{c|}{\multirow{2}{*}{$\frac{2*Recall*Prec}{Recall+Prec}$}} \\
%  & \multicolumn{3}{c|}{} \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[!htb]
% \caption {Evaluation metrics.}
% \label{table:metrics} 
% \begin{tabular}{|c|c|l|l|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{\textbf{Actual}} \\ \cline{3-4} 
% \multicolumn{2}{|c|}{} & yes & no \\ \hline
% \multirow{2}{*}{\textbf{Predicted}} & yes & TP & FP \\ \cline{2-4} 
%  & no & FN & TN \\ \hline
% \multirow{2}{*}{\textbf{Recall}} & \multicolumn{3}{c|}{\multirow{2}{*}{$\frac{TP}{TP+FN}$}} \\
%  & \multicolumn{3}{c|}{} \\ \hline
% % \multirow{2}{*}{\textbf{Precision}} & \multicolumn{3}{c|}{\multirow{2}{*}{$\frac{TP}{TP+FP}$}} \\
% %  & \multicolumn{3}{c|}{} \\ 
% % \multirow{2}{*}{\textbf{F-measure}} & \multicolumn{3}{c|}{\multirow{2}{*}{$\frac{2*Recall*Prec}{Recall+Prec}$}} \\
% %  & \multicolumn{3}{c|}{} \\ \hline
% \end{tabular}
% \end{table}

\subsection{Machine Learning Algorithms}
Five machine learning learners are selected as FARSEC, i.e., Random Forest, Naive Bayes, Logistic Regression, Multilayer Perceptron and K Nearest Neighbour. They are widely used in the classification problems~\cite{lessmann2008benchmarking}. We now give a brief description of each algorithm.

\textbf{Random Forest.} Random forests~\cite{liaw2002classification} have gained huge popularity in applications of machine learning during the last decades due to their good classification performance, scalability, and ease of use. Intuitively, a random forest can be considered as an ensemble of decision trees. The idea behind ensemble learning is to combine weak learners to build a more robust model, a strong learner, that has a better generalization error and is less susceptible to over-fitting. There are several advantages of random forest, e.g. it can be used for both classification and regression problems, and it is easy to measure the relative importance of each feature on the prediction.

\textbf{Naive Bayes.} Naive Bayes~\cite{rish2001empirical} is a very popular classifier for document classification, e.g., e-mail spam filtering. Naive Bayes is a subset of Bayesian decision theory, since the formulation makes some naive assumptions, this is what it meant by naive in the Naive Bayes classifier. Naive Bayes classifiers are computationally efficient and tend to perform well on relatively small datasets and is able to handle multiple classes compared to other algorithms.

\textbf{Logistic Regression.} Logistic regression~\cite{hosmer2013applied} is a classification model that works well on linearly separable classes, and it is one of the most widely used algorithm for classification in industry (e.g., weather forecasting). In general, logistic regression could be viewed as a probability estimation. A threshold can be set to predict the class a data belongs. Based upon the threshold, the obtained estimated probability is classified into classes. The decision boundary of logistic regression can be linear or non-linear. 

\textbf{Multilayer Perceptron.} Multilayer perceptron~\cite{gardner1998artificial} is an artificial neural network which is composed by multiple perceptrons. A perceptron is a single neuron model that is a precursor to larger neural networks. An input layer receives the signal and an output layer makes the prediction about the input. Between the input layer and the output layer, an arbitrary number of hidden layers act as the computational engine. In a sense, multilayer perceptron learns a mapping of the input training data, and best relate it to the predicted output. 

\textbf{K Nearest Neighbor.} K nearest neighbor classifier~\cite{keller1985fuzzy} is one of the simplest predictive model. When classifying a new element, nearest neighbor classifier checks in the training data for K objects close to the element (i.e., K nearest neighbors). The classifier returns the class by majority voting among its neighbors. K nearest neighbor is a typical ``lazy learner'' since it does not learn a discriminative function from the training data but just memorizes the training data instead. 


\begin{table*}[!htbp]
\caption {List of hyper-parameters tuned in different learners.}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|c|c|l}
\hline
\rowcolor[HTML]{EFEFEF}
\textbf{Learner} & \multicolumn{1}{c|}{\textbf{Parameters}} & \textbf{Default} & \textbf{Tuning Range} & \multicolumn{1}{c}{\textbf{Description}} \\ \hline
\multirow{6}{*}{Random Forest} & n\_estimators & 10 & {[}10,150{]} & The number of trees in the forest. \\ 
 & min\_samples\_leaf & 1 & {[}1,20{]} & The minimum number of samples required to be at a leaf node. \\  
 & min\_samples\_split & 2 & {[}2,20{]} & The minimum number of samples required to split an internal node. \\ 
 & max\_leaf\_nodes & None & {[}2,50{]} & Grow trees with  max\_leaf\_nodes in best-first fashion. \\  
 & max\_features & auto & {[}0.01,1{]} & The number of features to consider when looking for the best split \\  
 & max\_depth & None & {[}1,10{]} & The maximum depth of the tree. \\ \hline
\multirow{3}{*}{Logistic Regression} & C & 1.0 & {[}1.0,10.0{]} & Inverse of regularization strength. \\  
 & max\_iter & 100 & {[}50,200{]} & Useful only for the newton-cg, sag and lbfgs solvers. \\  
 & verbose & 0 & {[}0,10{]} & For the liblinear and lbfgs solvers set verbose to any positive number for verbosity. \\ \hline
\multirow{6}{*}{Multilayer Perceptron} & alpha & 0.0001 & {[}0.0001,0.001{]} & L2 penalty (regularization term) parameter. \\  
 & learning\_rate\_init & 0.001 & {[}0.001,0.01{]} & The initial learning rate used. \\
 & power\_t & 0.5 & {[}0.1,1{]} & The exponent for inverse scaling learning rate. \\
 & max\_iter & 200 & {[}50,300{]} & Maximum number of iterations. \\ 
 & momentum & 0.9 & {[}0.1,1{]} & Momentum for gradient descent update. \\ 
 & n\_iter\_no\_change & 10 & {[}1,100{]} & Maximum number of epochs to not meet tol improvement. \\ \hline
\multirow{2}{*}{K Nearest Neighbor} & leaf\_size & 30 & {[}10,100{]} & Leaf size passed to BallTree or KDTree. \\  
 & n\_neighbors & 5 & {[}1,10{]} & Number of neighbors to use by default for kneighbors queries. \\ \hline
Naive Bayes & var\_smoothing & 1e-9 & [0.0,1.0] & Portion of the largest variance of all features that is added to variances for calculation stability. \\ \hline
\end{tabular}
}
\label{table:hyperparameter}
\end{table*}


\subsection{Hyperparameter Tuning Range of Learners}

We implement our hyperparameter optimization techniques in scikit-learn. We choose scikit-learn because it integrates well-defined prediction learners as well as many configuration that we can choose. We select a group of hyperparameters for each learners in scikit-learn for the purpose of tuning. Table~\ref{table:hyperparameter} lists all the hyperparameters we select. We choose these ``tuning range'' for several reasons: (1) These ranges include the default value. (2) We could achieve a large gains in performance of our defect predictors by exploring these ranges. (3) These ranges are sufficient in tuning for this work.

% \begin{table*}[!htb]
% \caption {Comparison of Evaluation Results with DE tuning algorithm.}
% \begin{threeparttable}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|l|c|r|r|r|r|r|c|r|r|r|r|r|c|r|r|r|r|r|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \cellcolor[HTML]{EFEFEF} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{6}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DE3}} & \multicolumn{6}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DE10}} & \multicolumn{6}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{DE20}} \\ \cline{3-20} 
% \rowcolor[HTML]{EFEFEF} 
% \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Target}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Filter}}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{prec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{G}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{prec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{G}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{prec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{G}} \\ \hline
%  & train & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 \\ \cline{2-20} 
%  & \cellcolor[HTML]{EFEFEF}farsecsq & RF & 48.7 & 1.4 & 16.5 & 24.7 & 65.2 & RF & 48.7 & 1.3 & 17.7 & 25.9 & 65.2 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}53.0 & \cellcolor[HTML]{EFEFEF}1.4 & \cellcolor[HTML]{EFEFEF}17.2 & \cellcolor[HTML]{EFEFEF}26.0 & \cellcolor[HTML]{EFEFEF}68.9 \\ 
%  & farsectwo & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 333. & 21.3 & 27.1 \\ 
%  & farsec & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 \\  
%  & clni & LR & 14.8 & 0.1 & 35.4 & 20.9 & 25.8 & LR & 14.8 & 0.1 & 35.4 & 20.9 & 25.8 & LR & 14.8 & 0.1 & 35.4 & 20.9 & 25.8 \\  
%  & clnifarsecsq & RF & 47.8 & 1.4 & 15.8 & 23.7 & 64.4 & RF & 47.8 & 1.4 & 15.8 & 23.7 & 64.4 & RF & 49.6 & 1.4 & 16.3 & 24.6 & 66.0 \\ 
%  & clnifarsectwo & MP & 15.7 & 0.1 & 46.2 & 23.4 & 27.1 & MP & 16.5 & 0.1 & 40.4 & 23.5 & 28.4 & MP & 16.5 & 0.1 & 40.4 & 23.5 & 28.4 \\  
% \multirow{-8}{*}{Chromium} & clnifarsec & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 & LR & 15.7 & 0.2 & 33.3 & 21.3 & 27.1 \\ \hline
%  & train & MP & 33.3 & 10.7 & 3.6 & 6.6 & 48.5 & MP & 16.7 & 2.0 & 9.1 & 11.8 & 28.5 & MP & 16.7 & 0.2 & 50.0 & 25.0 & 28.6 \\ 
%  & farsecsq & NB & 16.7 & 6.7 & 2.9 & 5.0 & 28.3 & NB & 16.7 & 6.7 & 2.9 & 5.0 & 28.3 & NB & 16.7 & 6.7 & 2.9 & 5.0 & 28.3 \\  
%  & farsectwo & MP & 16.7 & 5.9 & 3.3 & 5.6 & 28.3 & MP & 16.7 & 5.9 & 3.3 & 5.6 & 28.3 & MP & 16.7 & 5.9 & 3.3 & 5.6 & 28.3 \\  
%  & \cellcolor[HTML]{EFEFEF}farsec & NB & 66.7 & 25.3 & 3.1 & 5.9 & 70.5 & NB & 66.7 & 25.3 & 3.1 & 5.9 & 70.5 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & \cellcolor[HTML]{EFEFEF}25.3 & \cellcolor[HTML]{EFEFEF}3.1 & \cellcolor[HTML]{EFEFEF}5.9 & \cellcolor[HTML]{EFEFEF}70.5 \\  
%  & clni & MP & 16.7 & 3.8 & 5.0 & 7.7 & 28.4 & MP & 16.7 & 3.8 & 5.0 & 7.7 & 28.4 & MP & 16.7 & 1.8 & 10.0 & 12.5 & 28.5 \\
%  & clnifarsecsq & NB & 16.7 & 8.5 & 2.3 & 4.1 & 28.2 & NB & 16.7 & 8.5 & 2.3 & 4.1 & 28.2 & NB & 16.7 & 8.5 & 2.3 & 4.1 & 28.2 \\ 
%  & clnifarsectwo & MP & 16.7 & 6.3 & 3.1 & 5.3 & 28.3 & MP & 16.7 & 6.3 & 3.1 & 5.3 & 28.3 & MP & 16.7 & 6.3 & 3.1 & 5.3 & 28.3 \\ 
% \multirow{-8}{*}{Wicket} & clnifarsec & MP & 16.7 & 0.2 & 50.0 & 25.0 & 28.6 & MP & 16.7 & 0.2 & 50.0 & 25.0 & 28.6 & MP & 16.7 & 0.2 & 50.0 & 25.0 & 28.6 \\ \hline
%  & train & MP & 28.6 & 0.6 & 40.0 & 33.3 & 44.4 & MP & 28.6 & 0.6 & 40.0 & 33.3 & 44.4 & MP & 28.6 & 0.6 & 40.0 & 33.3 & 44.4 \\  
%  & farsecsq & RF & 57.1 & 2.6 & 23.5 & 33.3 & 72.0 & RF & 57.1 & 2.2 & 26.7 & 36.4 & 72.1 & RF & 57.1 & 2.0 & 28.6 & 38.1 & 72.2 \\ 
%  & farsectwo & RF & 57.1 & 2.8 & 22.2 & 32.0 & 72.0 & RF & 57.1 & 2.8 & 22.2 & 32.0 & 72.0 & RF & 57.1 & 2.8 & 22.2 & 32.0 & 72.0 \\ 
%  & farsec & RF & 57.1 & 2.2 & 26.7 & 36.4 & 72.1 & RF & 57.1 & 2.2 & 26.7 & 36.4 & 72.1 & RF & 57.1 & 1.8 & 30.8 & 40.0 & 72.2 \\  
%  & clni & MP & 28.6 & 0.6 & 40.0 & 33.3 & 44.4 & MP & 28.6 & 0.6 & 40.0 & 33.3 & 44.4 & MP & 28.6 & 0.6 & 40.0 & 33.3 & 44.4 \\ 
%  & \cellcolor[HTML]{EFEFEF}clnifarsecsq & RF & 57.1 & 2.4 & 25.0 & 34.7 & 72.1 & RF & 57.1 & 1.6 & 33.3 & 42.1 & 72.3 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & \cellcolor[HTML]{EFEFEF}1.2 & \cellcolor[HTML]{EFEFEF}40.0 & \cellcolor[HTML]{EFEFEF}47.1 & \cellcolor[HTML]{EFEFEF}72.4 \\  
%  & clnifarsectwo & RF & 57.1 & 2.8 & 22.2 & 32.0 & 72.0 & RF & 57.1 & 2.6 & 23.5 & 33.3 & 72.0 & RF & 57.1 & 2.6 & 23.5 & 33.3 & 72.0 \\ 
% \multirow{-8}{*}{Ambari} & clnifarsec & RF & 57.1 & 2.2 & 26.7 & 36.3 & 72.1 & RF & 57.1 & 1.8 & 30.8 & 40.0 & 72.2 & RF & 57.1 & 1.6 & 33.3 & 42.1 & 72.3 \\ \hline
%  & train & LR & 11.1 & 2.1 & 16.7 & 13.3 & 20.0 & LR & 11.1 & 2.1 & 16.7 & 13.3 & 20.0 & MP & 16.7 & 1.7 & 27.3 & 20.7 & 28.5 \\ 
%  & farsecsq & RF & 22.2 & 6.0 & 12.1 & 15.7 & 35.9 & RF & 27.8 & 5.6 & 15.6 & 20.0 & 42.9 & RF & 27.8 & 5.3 & 16.1 & 20.4 & 42.9 \\ 
%  & farsectwo & MP & 72.2 & 39.6 & 6.4 & 11.7 & 65.8 & MP & 38.9 & 13.7 & 9.6 & 15.4 & 53.6 & MP & 33.3 & 7.0 & 15.0 & 20.7 & 49.1 \\ 
%  & farsec & MP & 11.1 & 1.5 & 22.2 & 14.8 & 20.0 & MP & 11.1 & 0.8 & 33.3 & 16.7 & 20.0 & MP & 11.1 & 0.6 & 40.0 & 17.4 & 20.0 \\ 
%  & clni & MP & 16.7 & 1.2 & 33.3 & 22.2 & 28.5 & MP & 16.7 & 1.2 & 33.3 & 22.2 & 28.5 & MP & 16.7 & 1.2 & 33.3 & 22.2 & 28.5 \\ 
%  & \cellcolor[HTML]{EFEFEF}clnifarsecsq & RF & 38.9 & 13.7 & 9.6 & 15.4 & 53.6 & RF & 38.9 & 13.5 & 9.7 & 15.6 & 53.7 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}38.9 & \cellcolor[HTML]{EFEFEF}8.7 & \cellcolor[HTML]{EFEFEF}14.3 & \cellcolor[HTML]{EFEFEF}20.9 & \cellcolor[HTML]{EFEFEF}54.5 \\ 
%  & clnifarsectwo & RF & 11.1 & 0.2 & 66.7 & 19.0 & 20.0 & RF & 16.7 & 0.6 & 50.0 & 25.0 & 28.5 & RF & 16.7 & 0.6 & 50.0 & 25.0 & 28.5 \\
% \multirow{-8}{*}{Camel} & clnifarsec & MP & 11.1 & 0.6 & 40.0 & 17.4 & 20.0 & MP & 11.1 & 0.6 & 40.0 & 17.4 & 20.0 & MP & 16.7 & 1.2 & 33.3 & 22.2 & 28.5 \\ \hline
%  & train & RF & 28.6 & 0.7 & 80.0 & 42.1 & 44.4 & RF & 28.5 & 0.4 & 85.7 & 42.9 & 44.4 & MP & 33.3 & 1.5 & 66.7 & 44.4 & 49.8 \\ 
%  & farsecsq & KNN & 59.5 & 40.6 & 11.8 & 19.8 & 59.5 & KNN & 59.5 & 40.6 & 11.8 & 19.8 & 59.5 & KNN & 59.5 & 40.6 & 11.8 & 19.8 & 59.5 \\  
%  & farsectwo & RF & 50.0 & 17.2 & 21.0 & 29.6 & 62.3 & RF & 50.0 & 17.2 & 21.0 & 29.6 & 62.3 & RF & 45.2 & 10.9 & 27.5 & 34.2 & 60.0 \\ 
%  & farsec & LR & 38.1 & 2.4 & 59.3 & 46.4 & 54.8 & LR & 38.1 & 2.4 & 59.3 & 46.4 & 54.8 & LR & 40.5 & 2.6 & 58.6 & 47.9 & 57.2 \\  
%  & clni & RF & 31.0 & 8.7 & 76.5 & 44.1 & 47.2 & RF & 31.0 & 6.6 & 81.3 & 44.8 & 47.2 & RF & 33.3 & 6.6 & 82.4 & 47.5 & 49.9 \\ 
%  & \cellcolor[HTML]{EFEFEF}clnifarsecsq & KNN & 59.5 & 41.0 & 11.7 & 19.6 & 59.2 & KNN & 59.5 & 40.8 & 11.8 & 19.7 & 59.3 & \cellcolor[HTML]{EFEFEF}KNN & \cellcolor[HTML]{EFEFEF}59.5 & \cellcolor[HTML]{EFEFEF}40.6 & \cellcolor[HTML]{EFEFEF}11.8 & \cellcolor[HTML]{EFEFEF}19.8 & \cellcolor[HTML]{EFEFEF}59.5 \\ 
%  & clnifarsectwo & RF & 42.9 & 10.7 & 26.9 & 33.0 & 57.9 & RF & 42.9 & 10.7 & 26.9 & 33.0 & 57.9 & RF & 40.5 & 8.7 & 29.8 & 34.3 & 56.1 \\ 
% \multirow{-8}{*}{Derby} & clnifarsec & LR & 38.1 & 2.8 & 55.2 & 45.1 & 54.7 & RF & 33.3 & 6.6 & 82.4 & 47.5 & 49.9 & RF & 35.1 & 8.7 & 78.9 & 49.2 & 52.5 \\ \hline
% \end{tabular}
% }
% \begin{tablenotes}
%     \item[1] Abbreviation of learners: \textbf{LR} (Logistic Regression), \textbf{RF} (Random Forest), \textbf{MP} (Multilayer Perceptron), \textbf{NB} (Naive  Bayes), \textbf{KNN} (K Nearest Neighbor).
% \end{tablenotes}
% \end{threeparttable}
% \end{table*}






% \begin{table*}[!htb]
% \caption {Comparison of Evaluation Results without and with SMOTE Data Balancing.}
% \begin{threeparttable}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|l|c|r|r|r|r|r|c|r|r|r|r|r|c|r|r|r|r|r}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \cellcolor[HTML]{EFEFEF} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{6}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Without SMOTE}} & \multicolumn{6}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{With Default SMOTE}} & \multicolumn{6}{c}{\cellcolor[HTML]{EFEFEF}\textbf{With Tuned SMOTE}} \\ \cline{3-20} 
% \rowcolor[HTML]{EFEFEF} 
% \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Target}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{Filter}}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{prec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{G}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{prec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{G}} & \textbf{Learner} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pd}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{pf}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{prec}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{F}} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{G}} \\ \hline
%  & train & MP & 15.7 & 0.1 & 51.4 & 24.0 & 27.1 & NB & 79.1 & 23.2 & 1.8 & 3.6 & 77.9 & RF & 52.2 & 2.9 & 9.0 & 15.4 & 67.9 \\  
%  & farsecsq & RF & 37.4 & 0.7 & 21.4 & 27.2 & 54.3 & NB & 86.1 & 32.5 & 1.4 & 2.8 & 75.7 & RF & 56.5 & 6.0 & 5.0 & 9.1 & 70.6 \\  
%  & farsectwo & MP & 15.7 & 0.1 & 54.5 & 24.3 & 27.1 & RF & 80.9 & 25.8 & 1.7 & 3.3 & 77.4 & RF & 44.3 & 2.0 & 10.9 & 17.6 & 61.1 \\ 
%  & farsec & MP & 15.7 & 0.1 & 50.0 & 23.8 & 27.1 & RF & 73.0 & 17.5 & 2.3 & 4.4 & 77.5 & RF & 54.8 & 3.2 & 8.6 & 14.8 & 70.0 \\ 
%  & clni & MP & 13.9 & 0.1 & 53.3 & 22.1 & 24.4 & NB & 71.3 & 19.6 & 2.0 & 3.8 & 75.6 & RF & 44.3 & 3.1 & 7.4 & 12.7 & 60.9 \\ 
%  & \cellcolor[HTML]{EFEFEF}clnifarsecsq & MP & 57.4 & 7.7 & 3.9 & 7.3 & 70.8 & NB & 87.0 & 29.5 & 1.6 & 3.1 & 77.9 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}64.3 & \cellcolor[HTML]{EFEFEF}7.8 & \cellcolor[HTML]{EFEFEF}4.3 & \cellcolor[HTML]{EFEFEF}8.1 & \cellcolor[HTML]{EFEFEF}75.8 \\  
%  & clnifarsectwo & MP & 15.6 & 0.1 & 46.2 & 23.4 & 27.1 & NB & 71.3 & 16.1 & 2.4 & 4.6 & 77.1 & \cellcolor[HTML]{FFFFFF}RF & 52.2 & 3.2 & 8.3 & 14.4 & 67.8 \\ 
% \multirow{-8}{*}{Chromium} & clnifarsec & MP & 15.7 & 0.1 & 45.0 & 23.2 & 27.1 & NB & 65.2 & 18.6 & 1.9 & 3.7 & 72.4 & RF & 47.8 & 2.8 & 8.7 & 14.7 & 64.1 \\ \hline
%  & train & NB & 0.0 & 5.1 & 0.0 & 0.0 & 0.0 & NB & 50.0 & 26.7 & 2.2 & 4.3 & 59.4 & NB & 50.0 & 11.9 & 4.8 & 8.8 & 63.8 \\ 
%  & \cellcolor[HTML]{FFFFFF}farsecsq & NB & 83.3 & 66.8 & 1.5 & 2.9 & 47.5 & KNN & 16.7 & 5.3 & 3.7 & 6.1 & 28.3 & \cellcolor[HTML]{FFFFFF}NB & \cellcolor[HTML]{FFFFFF}83.3 & \cellcolor[HTML]{FFFFFF}66.8 & \cellcolor[HTML]{FFFFFF}1.5 & \cellcolor[HTML]{FFFFFF}2.9 & \cellcolor[HTML]{FFFFFF}47.5 \\ 
%  & farsectwo & NB & 66.7 & 61.5 & 1.3 & 2.5 & 48.8 & NB & 66.7 & 69.2 & 1.2 & 2.3 & 42.1 & NB & 66.7 & 62.6 & 1.3 & 2.5 & 50.0 \\  
%  & \cellcolor[HTML]{EFEFEF}farsec & NB & 66.7 & 23.1 & 3.4 & 6.5 & 71.4 & NB & 66.7 & 40.3 & 2.0 & 3.8 & 63.0 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & \cellcolor[HTML]{EFEFEF}23.1 & \cellcolor[HTML]{EFEFEF}3.4 & \cellcolor[HTML]{EFEFEF}6.5 & \cellcolor[HTML]{EFEFEF}71.4 \\ 
%  & clni & NB & 0.0 & 4.5 & 0.0 & 0.0 & 0.0 & NB & 33.3 & 23.3 & 1.7 & 3.3 & 46.5 & NB & 16.7 & 6.7 & 2.9 & 5.0 & 28.3 \\  
%  & clnifarsecsq & NB & 83.3 & 66.8 & 1.5 & 2.9 & 47.5 & NB & 83.3 & 66.8 & 1.5 & 2.9 & 47.5 & NB & 83.3 & 66.8 & 1.5 & 2.9 & 47.5 \\  
%  & clnifarsectwo & NB & 66.7 & 61.3 & 1.3 & 2.6 & 48.9 & NB & 66.7 & 61.3 & 1.3 & 2.6 & 48.9 & NB & 66.7 & 61.3 & 1.3 & 2.6 & 48.9 \\  
% \multirow{-8}{*}{Wicket} & \cellcolor[HTML]{FFFFFF}clnifarsec & NB & 66.7 & 23.1 & 3.4 & 6.5 & 71.4 & NB & 66.7 & 32.6 & 2.4 & 4.7 & 67.0 & \cellcolor[HTML]{FFFFFF}NB & \cellcolor[HTML]{FFFFFF}66.7 & \cellcolor[HTML]{FFFFFF}22.9 & \cellcolor[HTML]{FFFFFF}3.4 & \cellcolor[HTML]{FFFFFF}6.5 & \cellcolor[HTML]{FFFFFF}71.5 \\ \hline
%  & train & LR & 28.6 & 0.8 & 33.3 & 30.8 & 44.4 & LR & 57.1 & 16.6 & 4.7 & 8.6 & 67.8 & LR & 42.9 & 7.9 & 7.1 & 12.2 & 58.5 \\  
%  & farsecsq & RF & 42.9 & 7.3 & 7.7 & 13.0 & 58.6 & RF & 42.8 & 16.6 & 3.5 & 6.5 & 56.6 & RF & 57.1 & 16.0 & 4.8 & 8.9 & 6.8 \\  
%  & \cellcolor[HTML]{FFFFFF}farsectwo & \cellcolor[HTML]{FFFFFF}RF & \cellcolor[HTML]{FFFFFF}42.8 & \cellcolor[HTML]{FFFFFF}4.3 & \cellcolor[HTML]{FFFFFF}12.5 & \cellcolor[HTML]{FFFFFF}19.4 & \cellcolor[HTML]{FFFFFF}59.2 & RF & 57.1 & 10.3 & 7.2 & 12.9 & 69.8 & RF & 28.6 & 2.6 & 13.3 & 18.2 & 44.2 \\  
%  & farsec & MP & 28.6 & 2.0 & 16.7 & 21.1 & 44.2 & RF & 57.1 & 4.7 & 14.8 & 23.5 & 71.5 & RF & 28.6 & 1.4 & 22.2 & 25.0 & 44.3 \\ 
%  & clni & LR & 28.6 & 0.1 & 33.3 & 30.8 & 44.4 & RF & 57.1 & 2.6 & 23.5 & 33.3 & 72.0 & RF & 42.9 & 1.6 & 27.3 & 33.3 & 59.7 \\  
%  & \cellcolor[HTML]{FFFFFF}clnifarsecsq & RF & 57.1 & 14.2 & 5.4 & 9.9 & 68.6 & RF & 57.1 & 11.6 & 6.6 & 11.8 & 69.5 & \cellcolor[HTML]{FFFFFF}RF & \cellcolor[HTML]{FFFFFF}57.1 & \cellcolor[HTML]{FFFFFF}8.7 & \cellcolor[HTML]{FFFFFF}8.5 & \cellcolor[HTML]{FFFFFF}14.8 & \cellcolor[HTML]{FFFFFF}70.3 \\  
%  & \cellcolor[HTML]{EFEFEF}clnifarsectwo & RF & 42.9 & 3.4 & 15.0 & 22.2 & 59.4 & RF & 57.1 & 7.5 & 9.8 & 16.7 & 70.6 & \cellcolor[HTML]{EFEFEF}RF & \cellcolor[HTML]{EFEFEF}57.1 & \cellcolor[HTML]{EFEFEF}4.1 & \cellcolor[HTML]{EFEFEF}16.7 & \cellcolor[HTML]{EFEFEF}25.8 & \cellcolor[HTML]{EFEFEF}71.6 \\ 
% \multirow{-8}{*}{Ambari} & clnifarsec & LR & 28.5 & 2.8 & 12.5 & 17.4 & 44.2 & RF & 57.1 & 3.7 & 18.2 & 27.6 & 71.7 & RF & 42.9 & 1.2 & 33.3 & 37.5 & 59.8 \\ \hline
%  & train & NB & 16.7 & 10.8 & 5.5 & 8.2 & 28.1 & LR & 22.2 & 18.5 & 4.3 & 7.2 & 34.9 & LR & 22.2 & 9.8 & 7.8 & 11.6 & 35.7 \\  
%  & \cellcolor[HTML]{FFFFFF}farsecsq & RF & 38.9 & 17.6 & 7.6 & 12.7 & 52.8 & RF & 33.3 & 17.0 & 6.8 & 11.3 & 47.6 & \cellcolor[HTML]{FFFFFF}RF & \cellcolor[HTML]{FFFFFF}44.4 & \cellcolor[HTML]{FFFFFF}19.3 & \cellcolor[HTML]{FFFFFF}7.9 & \cellcolor[HTML]{FFFFFF}13.4 & \cellcolor[HTML]{FFFFFF}57.3 \\ 
%  & farsectwo & NB & 61.1 & 50.8 & 4.3 & 8.0 & 54.5 & RF & 22.2 & 5.0 & 14.3 & 17.4 & 36.0 & NB & 66.7 & 57.7 & 4.1 & 7.8 & 51.8 \\  
%  & farsec & NB & 22.2 & 12.4 & 6.3 & 9.8 & 35.4 & NB & 33.3 & 39.4 & 3.1 & 5.6 & 43.0 & NB & 22.2 & 11.2 & 6.9 & 10.5 & 35.5 \\ 
%  & clni & NB & 16.7 & 10.6 & 5.6 & 8.3 & 28.1 & NB & 38.9 & 36.9 & 3.8 & 6.9 & 48.1 & LR & 16.7 & 3.9 & 13.6 & 15.0 & 28.4 \\ 
%  & clnifarsecsq & NB & 83.3 & 78.4 & 3.8 & 7.3 & 34.3 & RF & 22.2 & 11.8 & 6.6 & 10.1 & 35.5 & RF & 33.3 & 16.6 & 7.0 & 11.5 & 47.6 \\ 
%  & \cellcolor[HTML]{EFEFEF}clnifarsectwo & NB & 61.1 & 50.0 & 4.4 & 8.1 & 55.0 & NB & 72.2 & 69.1 & 3.8 & 7.1 & 43.3 & \cellcolor[HTML]{EFEFEF}NB & \cellcolor[HTML]{EFEFEF}66.7 & \cellcolor[HTML]{EFEFEF}55.8 & \cellcolor[HTML]{EFEFEF}4.3 & \cellcolor[HTML]{EFEFEF}8.0 & \cellcolor[HTML]{EFEFEF}53.2 \\  
% \multirow{-8}{*}{Camel} & clnifarsec & NB & 22.2 & 11.6 & 6.7 & 10.3 & 35.5 & LR & 33.3 & 17.4 & 6.7 & 11.1 & 47.5 & LR & 22.2 & 5.4 & 13.3 & 16.7 & 36.0 \\ \hline
%  & train & NB & 45.2 & 3.5 & 54.3 & 49.4 & 61.6 & NB & 59.5 & 21.8 & 20.0 & 29.9 & 67.6 & NB & 50.0 & 3.7 & 55.3 & 52.5 & 65.8 \\  
%  & farsecsq & KNN & 35.7 & 26.0 & 11.2 & 17.0 & 48.2 & RF & 54.7 & 51.7 & 8.8 & 15.2 & 51.3 & RF & 66.7 & 53.1 & 10.3 & 17.9 & 55.1 \\  
%  & farsectwo & RF & 42.9 & 14.2 & 21.7 & 28.8 & 57.2 & RF & 54.7 & 25.3 & 16.5 & 25.4 & 63.2 & RF & 47.6 & 12.7 & 25.6 & 33.3 & 61.6 \\  
%  & farsec & NB & 47.6 & 4.1 & 51.3 & 49.4 & 63.6 & LR & 59.5 & 12.7 & 30.1 & 40.0 & 70.8 & LR & 42.9 & 3.9 & 50.0 & 46.2 & 59.3 \\ 
%  & \cellcolor[HTML]{EFEFEF}clni & NB & 45.2 & 3.5 & 54.3 & 49.4 & 61.6 & NB & 59.5 & 15.3 & 26.3 & 36.5 & 69.9 & \cellcolor[HTML]{EFEFEF}LR & \cellcolor[HTML]{EFEFEF}52.3 & \cellcolor[HTML]{EFEFEF}8.7 & \cellcolor[HTML]{EFEFEF}35.5 & \cellcolor[HTML]{EFEFEF}42.3 & \cellcolor[HTML]{EFEFEF}66.6 \\  
%  & clnifarsecsq & RF & 71.4 & 57.9 & 10.2 & 17.8 & 53.0 & RF & 76.2 & 74.7 & 8.6 & 15.4 & 38.0 & RF & 78.6 & 70.3 & 9.3 & 16.6 & 43.1 \\  
%  & clnifarsectwo & RF & 35.7 & 8.5 & 27.8 & 31.3 & 51.4 & RF & 52.4 & 26.2 & 15.5 & 23.9 & 61.3 & RF & 35.7 & 9.8 & 25.0 & 29.4 & 51.2 \\  
% \multirow{-8}{*}{Derby} & clnifarsec & NB & 47.6 & 3.9 & 52.6 & 50.0 & 63.7 & RF & 52.3 & 12.2 & 28.2 & 36.7 & 65.7 & NB & 47.6 & 3.7 & 54.1 & 50.6 & 63.7 \\ \hline
% \end{tabular}
% }
% \begin{tablenotes}
%     \item[1] Abbreviation of learners: \textbf{LR} (Logistic Regression), \textbf{RF} (Random Forest), \textbf{MP} (Multilayer Perceptron), \textbf{NB} (Naive  Bayes), \textbf{KNN} (K Nearest Neighbor).
% \end{tablenotes}
% \end{threeparttable}
% \end{table*}


% \begin{figure*}
% \renewcommand{\baselinestretch}{0.65} 
%  \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% \vspace{2.5mm}
% \begin{center}a. The recall results of project Chromium with FARSEC and CLNI filtering\end{center}
% \noindent \begin{tabular}{llrrc}
%   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% 1 &      clnifarsecsq\_NB &    68 &  0 & \quart{68}{0}{68}{100} \\     
% 1 &      farsecsq\_NB &    68 &  0 & \quart{68}{0}{68}{100} \\             
% 2 &      clnifarsecsq\_MP &    56 &  0 & \quart{56}{0}{56}{100} \\         
% 2 &      farsecsq\_MP &    56 &  0 & \quart{56}{0}{56}{100} \\             
% 3 &      clnifarsecsq\_LR &    49 &  0 & \quart{49}{0}{49}{100} \\         
% 3 &      farsecsq\_LR &    49 &  0 & \quart{49}{0}{49}{100} \\             
% 3 &      clni\_NB &    50 &  0 & \quart{50}{0}{50}{100} \\                 
% 3 &      clnifarsec\_NB &    50 &  0 & \quart{50}{0}{50}{100} \\           
% 3 &      farsec\_NB &    50 &  0 & \quart{50}{0}{50}{100} \\               
% 3 &      clnifarsectwo\_NB &    50 &  0 & \quart{50}{0}{50}{100} \\        
% 3 &      train\_NB &    50 &  0 & \quart{50}{0}{50}{100} \\                
% 3 &      farsectwo\_NB &    50 &  0 & \quart{50}{0}{50}{100} \\            
% 4 &      farsecsq\_RF &    27 &  11 & \quart{27}{11}{27}{100} \\           
% 4 &      clnifarsecsq\_RF &    38 &  5 & \quart{35}{5}{38}{100} \\          
% 5 &      clnifarsectwo\_MP &    14 &  0 & \quart{14}{0}{14}{100} \\         
% 5 &      train\_MP &    16 &  2 & \quart{14}{2}{16}{100} \\                 
% 5 &      farsectwo\_MP &    15 &  0 & \quart{15}{0}{15}{100} \\            
% 5 &      farsec\_MP &    15 &  1 & \quart{14}{1}{15}{100} \\               
% 5 &      clni\_MP &    15 &  1 & \quart{15}{1}{15}{100} \\                 
% 6 &      clnifarsecsq\_KNN &    10 &  0 & \quart{10}{0}{10}{100} \\        
% 6 &      farsecsq\_KNN &    10 &  0 & \quart{10}{0}{10}{100} \\            
% 6 &      clnifarsec\_LR &    11 &  0 & \quart{11}{0}{11}{100} \\           
% 6 &      clnifarsectwo\_LR &    11 &  0 & \quart{11}{0}{11}{100} \\        
% 6 &      clni\_LR &    11 &  0 & \quart{11}{0}{11}{100} \\                 
% 6 &      farsectwo\_LR &    12 &  0 & \quart{12}{0}{12}{100} \\             
% 6 &      farsec\_LR &    12 &  0 & \quart{12}{0}{12}{100} \\                
% 6 &      train\_LR &    12 &  0 & \quart{12}{0}{12}{100} \\                 
% 6 &      clnifarsec\_MP &    12 &  0 & \quart{12}{0}{12}{100} \\           
% 7 &      farsec\_RF &    3 &  1 & \quart{3}{1}{3}{100} \\                  
% 7 &      train\_RF &    4 &  1 & \quart{3}{1}{4}{100} \\                   
% 7 &      farsectwo\_RF &    4 &  1 & \quart{3}{1}{4}{100} \\               
% 7 &      clni\_RF &    4 &  2 & \quart{4}{2}{4}{100} \\                    
% 7 &      clnifarsec\_RF &    4 &  4 & \quart{4}{4}{4}{100} \\              
% 7 &      clnifarsectwo\_RF &    6 &  3 & \quart{5}{3}{6}{100} \\           
% 8 &      farsectwo\_KNN &    1 &  0 & \quart{1}{0}{1}{100} \\              
% 8 &      train\_KNN &    1 &  0 & \quart{1}{0}{1}{100} \\                  
% 8 &      clnifarsectwo\_KNN &    1 &  0 & \quart{1}{0}{1}{100} \\          
% 8 &      clni\_KNN &    1 &  0 & \quart{1}{0}{1}{100} \\                   
% 8 &      farsec\_KNN &    1 &  0 & \quart{1}{0}{1}{100} \\                 
% 8 &      clnifarsec\_KNN &    1 &  0 & \quart{1}{0}{1}{100} \\             
%     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %   1 & clnifarsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   1 &     farsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   2 &    farsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 & clnifarsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &       farsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &   clnifarsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   3 &         clni &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %   3 &        train &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   1 & farsectwo\_RF\_DE &    0.77  &  0.0 & \quart{79}{0}{79}{109} \\
% %   2 &    farsectwo &    0.56  &  0.42 & \quart{0}{53}{53}{109} \\
% %   2 & clnifarsectwo &    0.56  &  0.0 & \quart{53}{0}{53}{109} \\
% %   3 &         clni &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 & clnifarsecsq &    0.14  &  0.14 & \quart{0}{17}{0}{109} \\
% %   3 &        train &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 &     farsecsq &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %   3 &       farsec &    0.28  &  0.0 & \quart{17}{0}{17}{109} \\
% %   3 &   clnifarsec &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %   1 &       farsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\
% %   1 &   clnifarsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\ 
% %   2 &         clni &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &        train &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &     farsecsq &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   3 & clnifarsecsq &    0.11  &  0.0 & \quart{24}{0}{24}{469} \\
% %   4 &    farsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %   4 & clnifarsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %   1 & farsectwo\_RF\_DE &    0.68  &  0.0 & \quart{79}{0}{79}{132} \\
% %   2 & clnifarsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   2 &     farsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   3 &       farsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   3 &   clnifarsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   4 &        train &    0.45  &  0.0 & \quart{42}{0}{42}{132} \\
% %   5 & clnifarsectwo &    0.38  &  0.05 & \quart{22}{9}{31}{132} \\
% %   5 &    farsectwo &    0.43  &  0.05 & \quart{34}{8}{39}{132} \\
% %   6 &         clni &    0.21  &  0.05 & \quart{0}{8}{3}{132} \\



%  %%% ----END HERE---------------------------------
%   \end{tabular}} \end{minipage}}\hspace{12mm}
% \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% % \begin{center}b. TPP results wit FARSEC and CLNI filtering\end{center}

% % \noindent \begin{tabular}{llrrc}
% %   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% %   \nm{Chromium}\\
% %  \rowcolor{gray!20}   1* &      train &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec &    69 &  18 & \quart{69}{18}{76}{100} \\
% %  \rowcolor{gray!20}   1* &      train\_DE &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq\_DE &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo\_DE &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec\_DE &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni\_DE &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq\_DE &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     \\
% %     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %     1 &      train &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo &    178 &  122 & \ofr \\
% %     4 &      clnifarsec &    178 &  122 & \ofr \\
% %     1 &      train\_DE &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq\_DE &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo\_DE &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq\_DE &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo\_DE &    178 &  122 & \ofr \\
% %     4 &      clnifarsec\_DE &    178 &  122 & \ofr \\
% %     \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   \rowcolor{gray!20}   1* &      train &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec &    56 &  33 & \quart{38}{33}{56}{100} \\
% %   \rowcolor{gray!20}   1* &      train\_DE &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq\_DE &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo\_DE &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec\_DE &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni\_DE &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq\_DE &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %     \rowcolor{gray!20}   1* &      train &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq\_DE &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo\_DE &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec\_DE &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni\_DE &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq\_DE &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo\_DE &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec\_DE &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %     \rowcolor{gray!20}   1* &      train &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec &    99 &  444 & \ofr \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq\_DE &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo\_DE &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec\_DE &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni\_DE &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq\_DE &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo\_DE &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec\_DE &    99 &  444 & \ofr \\

% %   %%% ----END HERE----------------------------------
   
   
% %   \end{tabular}
%   }

% \end{minipage}
% }
%  \caption{
% \%  WPP and TPP precision results of using default hyperparameter in scikit-learn and tuning using differential evolutionary (DE) algorithm
%   }
%  \label{fig:jur}
% \end{figure*}


% \begin{figure*}
% \renewcommand{\baselinestretch}{0.65} 
%  \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% \vspace{2.5mm}
% \begin{center}a. The recall results of project Wicket with FARSEC and CLNI filtering\end{center}
% \noindent \begin{tabular}{llrrc}
%   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
%     1 &      clnifarsecsq\_NB &    83 &  0 & \quart{83}{0}{83}{100} \\
%     1 &      farsecsq\_NB &    83 &  0 & \quart{83}{0}{83}{100} \\
%     2 &      clnifarsec\_NB &    67 &  0 & \quart{67}{0}{67}{100} \\
%     2 &      farsec\_NB &    67 &  0 & \quart{67}{0}{67}{100} \\
%     2 &      clnifarsectwo\_NB &    67 &  0 & \quart{67}{0}{67}{100} \\
%     2 &      farsectwo\_NB &    67 &  0 & \quart{67}{0}{67}{100} \\
%     3 &      train\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsectwo\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsecsq\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsectwo\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsecsq\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsectwo\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clni\_NB &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsec\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_RF\_DE3 &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsectwo\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsec\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clni\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsectwo\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clni\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_NB &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clni\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsecsq\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsecsq\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_MP\_DE3 &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      train\_KNN\_DE3 &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsecsq\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsecsq\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsecsq\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsectwo\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsec\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsecsq\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsec\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsectwo\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsec\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsectwo\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      farsec\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsec\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clnifarsec\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\
%     3 &      clni\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\
%     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %   1 & clnifarsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   1 &     farsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   2 &    farsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 & clnifarsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &       farsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &   clnifarsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   3 &         clni &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %   3 &        train &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   1 & farsectwo\_RF\_DE &    0.77  &  0.0 & \quart{79}{0}{79}{109} \\
% %   2 &    farsectwo &    0.56  &  0.42 & \quart{0}{53}{53}{109} \\
% %   2 & clnifarsectwo &    0.56  &  0.0 & \quart{53}{0}{53}{109} \\
% %   3 &         clni &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 & clnifarsecsq &    0.14  &  0.14 & \quart{0}{17}{0}{109} \\
% %   3 &        train &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 &     farsecsq &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %   3 &       farsec &    0.28  &  0.0 & \quart{17}{0}{17}{109} \\
% %   3 &   clnifarsec &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %   1 &       farsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\
% %   1 &   clnifarsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\ 
% %   2 &         clni &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &        train &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &     farsecsq &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   3 & clnifarsecsq &    0.11  &  0.0 & \quart{24}{0}{24}{469} \\
% %   4 &    farsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %   4 & clnifarsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %   1 & farsectwo\_RF\_DE &    0.68  &  0.0 & \quart{79}{0}{79}{132} \\
% %   2 & clnifarsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   2 &     farsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   3 &       farsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   3 &   clnifarsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   4 &        train &    0.45  &  0.0 & \quart{42}{0}{42}{132} \\
% %   5 & clnifarsectwo &    0.38  &  0.05 & \quart{22}{9}{31}{132} \\
% %   5 &    farsectwo &    0.43  &  0.05 & \quart{34}{8}{39}{132} \\
% %   6 &         clni &    0.21  &  0.05 & \quart{0}{8}{3}{132} \\



%  %%% ----END HERE---------------------------------
%   \end{tabular}} \end{minipage}}\hspace{12mm}
% \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% % \begin{center}b. TPP results wit FARSEC and CLNI filtering\end{center}

% % \noindent \begin{tabular}{llrrc}
% %   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% %   \nm{Chromium}\\
% %  \rowcolor{gray!20}   1* &      train &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec &    69 &  18 & \quart{69}{18}{76}{100} \\
% %  \rowcolor{gray!20}   1* &      train\_DE &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq\_DE &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo\_DE &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec\_DE &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni\_DE &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq\_DE &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     \\
% %     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %     1 &      train &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo &    178 &  122 & \ofr \\
% %     4 &      clnifarsec &    178 &  122 & \ofr \\
% %     1 &      train\_DE &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq\_DE &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo\_DE &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq\_DE &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo\_DE &    178 &  122 & \ofr \\
% %     4 &      clnifarsec\_DE &    178 &  122 & \ofr \\
% %     \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   \rowcolor{gray!20}   1* &      train &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec &    56 &  33 & \quart{38}{33}{56}{100} \\
% %   \rowcolor{gray!20}   1* &      train\_DE &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq\_DE &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo\_DE &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec\_DE &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni\_DE &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq\_DE &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %     \rowcolor{gray!20}   1* &      train &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq\_DE &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo\_DE &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec\_DE &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni\_DE &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq\_DE &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo\_DE &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec\_DE &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %     \rowcolor{gray!20}   1* &      train &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec &    99 &  444 & \ofr \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq\_DE &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo\_DE &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec\_DE &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni\_DE &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq\_DE &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo\_DE &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec\_DE &    99 &  444 & \ofr \\

% %   %%% ----END HERE----------------------------------
   
   
% %   \end{tabular}
%   }

% \end{minipage}
% }
%  \caption{
% \%  WPP and TPP precision results of using default hyperparameter in scikit-learn and tuning using differential evolutionary (DE) algorithm
%   }
%  \label{fig:jur}
% \end{figure*}


% \begin{figure*}
% \renewcommand{\baselinestretch}{0.65} 
%  \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% \vspace{2.5mm}
% \begin{center}a. The recall results of project Ambari with FARSEC and CLNI filtering\end{center}
% \noindent \begin{tabular}{llrrc}
%   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
%  1 &      clnifarsecsq\_NB &    86 &  0 & \quart{86}{0}{86}{100} \\    
% 1 &      farsecsq\_NB &    86 &  0 & \quart{86}{0}{86}{100} \\        
% 2 &      clnifarsectwo\_NB &    71 &  0 & \quart{71}{0}{71}{100} \\   
% 2 &      farsectwo\_NB &    71 &  0 & \quart{71}{0}{71}{100} \\       
% 3 &      clnifarsecsq\_LR &    56 &  0 & \quart{56}{0}{56}{100} \\    
% 4 &      clnifarsecsq\_RF &    43 &  14 & \quart{28}{14}{43}{100} \\  
% 4 &      clnifarsectwo\_LR &    43 &  0 & \quart{43}{0}{43}{100} \\   
% 4 &      farsecsq\_RF &    43 &  13 & \quart{43}{13}{43}{100} \\      
% 5 &      farsectwo\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\       
% 5 &      farsec\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\          
% 5 &      clnifarsec\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\      
% 5 &      clni\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\            
% 5 &      train\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\           
% 5 &      farsecsq\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\        
% 5 &      clnifarsecsq\_MP &    28 &  0 & \quart{28}{0}{28}{100} \\    
% 5 &      farsectwo\_MP &    28 &  0 & \quart{28}{0}{28}{100} \\       
% 5 &      farsec\_MP &    28 &  14 & \quart{14}{14}{28}{100} \\        
% 5 &      farsecsq\_MP &    28 &  0 & \quart{28}{0}{28}{100} \\        
% 5 &      clnifarsectwo\_RF &    28 &  42 & \quart{14}{42}{28}{100} \\ 
% 5 &      clnifarsectwo\_MP &    28 &  14 & \quart{14}{14}{28}{100} \\ 
% 6 &      farsectwo\_KNN &    14 &  0 & \quart{14}{0}{14}{100} \\      
% 6 &      clnifarsectwo\_KNN &    14 &  0 & \quart{14}{0}{14}{100} \\  
% 6 &      train\_MP &    14 &  0 & \quart{14}{0}{14}{100} \\           
% 6 &      clni\_NB &    14 &  0 & \quart{14}{0}{14}{100} \\            
% 6 &      farsectwo\_RF &    14 &  28 & \quart{0}{28}{14}{100} \\      
% 6 &      clnifarsec\_NB &    14 &  0 & \quart{14}{0}{14}{100} \\      
% 6 &      farsec\_NB &    14 &  0 & \quart{14}{0}{14}{100} \\          
% 6 &      train\_NB &    14 &  0 & \quart{14}{0}{14}{100} \\           
% 6 &      clnifarsecsq\_KNN &    14 &  0 & \quart{14}{0}{14}{100} \\   
% 6 &      farsecsq\_KNN &    14 &  0 & \quart{14}{0}{14}{100} \\       
% 6 &      clnifarsec\_MP &    14 &  0 & \quart{14}{0}{14}{100} \\      
% 7 &      train\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\              
% 7 &      train\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\             
% 7 &      clni\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\               
% 7 &      clni\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\              
% 7 &      farsec\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\             
% 7 &      farsec\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\            
% 7 &      clnifarsec\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\        
% 7 &      clnifarsec\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\         
% 7 &      clni\_MP &    0 &  14 & \quart{0}{14}{0}{100} \\             
%     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %   1 & clnifarsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   1 &     farsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   2 &    farsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 & clnifarsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &       farsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &   clnifarsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   3 &         clni &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %   3 &        train &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   1 & farsectwo\_RF\_DE &    0.77  &  0.0 & \quart{79}{0}{79}{109} \\
% %   2 &    farsectwo &    0.56  &  0.42 & \quart{0}{53}{53}{109} \\
% %   2 & clnifarsectwo &    0.56  &  0.0 & \quart{53}{0}{53}{109} \\
% %   3 &         clni &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 & clnifarsecsq &    0.14  &  0.14 & \quart{0}{17}{0}{109} \\
% %   3 &        train &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 &     farsecsq &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %   3 &       farsec &    0.28  &  0.0 & \quart{17}{0}{17}{109} \\
% %   3 &   clnifarsec &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %   1 &       farsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\
% %   1 &   clnifarsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\ 
% %   2 &         clni &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &        train &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &     farsecsq &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   3 & clnifarsecsq &    0.11  &  0.0 & \quart{24}{0}{24}{469} \\
% %   4 &    farsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %   4 & clnifarsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %   1 & farsectwo\_RF\_DE &    0.68  &  0.0 & \quart{79}{0}{79}{132} \\
% %   2 & clnifarsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   2 &     farsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   3 &       farsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   3 &   clnifarsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   4 &        train &    0.45  &  0.0 & \quart{42}{0}{42}{132} \\
% %   5 & clnifarsectwo &    0.38  &  0.05 & \quart{22}{9}{31}{132} \\
% %   5 &    farsectwo &    0.43  &  0.05 & \quart{34}{8}{39}{132} \\
% %   6 &         clni &    0.21  &  0.05 & \quart{0}{8}{3}{132} \\



%  %%% ----END HERE---------------------------------
%   \end{tabular}} \end{minipage}}\hspace{12mm}
% \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% % \begin{center}b. TPP results wit FARSEC and CLNI filtering\end{center}

% % \noindent \begin{tabular}{llrrc}
% %   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% %   \nm{Chromium}\\
% %  \rowcolor{gray!20}   1* &      train &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec &    69 &  18 & \quart{69}{18}{76}{100} \\
% %  \rowcolor{gray!20}   1* &      train\_DE &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq\_DE &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo\_DE &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec\_DE &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni\_DE &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq\_DE &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     \\
% %     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %     1 &      train &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo &    178 &  122 & \ofr \\
% %     4 &      clnifarsec &    178 &  122 & \ofr \\
% %     1 &      train\_DE &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq\_DE &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo\_DE &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq\_DE &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo\_DE &    178 &  122 & \ofr \\
% %     4 &      clnifarsec\_DE &    178 &  122 & \ofr \\
% %     \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   \rowcolor{gray!20}   1* &      train &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec &    56 &  33 & \quart{38}{33}{56}{100} \\
% %   \rowcolor{gray!20}   1* &      train\_DE &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq\_DE &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo\_DE &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec\_DE &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni\_DE &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq\_DE &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %     \rowcolor{gray!20}   1* &      train &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq\_DE &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo\_DE &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec\_DE &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni\_DE &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq\_DE &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo\_DE &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec\_DE &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %     \rowcolor{gray!20}   1* &      train &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec &    99 &  444 & \ofr \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq\_DE &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo\_DE &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec\_DE &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni\_DE &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq\_DE &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo\_DE &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec\_DE &    99 &  444 & \ofr \\

% %   %%% ----END HERE----------------------------------
   
   
% %   \end{tabular}
%   }

% \end{minipage}
% }
%  \caption{
% \%  WPP and TPP precision results of using default hyperparameter in scikit-learn and tuning using differential evolutionary (DE) algorithm
%   }
%  \label{fig:jur}
% \end{figure*}



% \begin{figure*}
% \renewcommand{\baselinestretch}{0.65} 
%  \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% \vspace{2.5mm}
% \begin{center}a. The recall results of project Camel with FARSEC and CLNI filtering\end{center}
% \noindent \begin{tabular}{llrrc}
%   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% 1 &      clnifarsecsq\_NB &    83 &  0 & \quart{83}{0}{83}{100} \\
% 1 &      farsecsq\_NB &    83 &  0 & \quart{83}{0}{83}{100} \\             
% 2 &      clnifarsectwo\_NB &    61 &  0 & \quart{61}{0}{61}{100} \\        
% 2 &      farsectwo\_NB &    61 &  0 & \quart{61}{0}{61}{100} \\            
% 3 &      clnifarsecsq\_RF &    22 &  11 & \quart{17}{11}{22}{100} \\       
% 3 &      clnifarsec\_NB &    22 &  0 & \quart{22}{0}{22}{100} \\           
% 3 &      farsec\_NB &    22 &  0 & \quart{22}{0}{22}{100} \\               
% 3 &      farsecsq\_RF &    22 &  6 & \quart{22}{6}{22}{100} \\             
% 4 &      clnifarsecsq\_LR &    17 &  0 & \quart{17}{0}{17}{100} \\         
% 4 &      clni\_NB &    17 &  0 & \quart{17}{0}{17}{100} \\                 
% 4 &      train\_NB &    17 &  0 & \quart{17}{0}{17}{100} \\                
% 4 &      farsecsq\_LR &    17 &  0 & \quart{17}{0}{17}{100} \\             
% 5 &      clnifarsecsq\_MP &    11 &  0 & \quart{11}{0}{11}{100} \\         
% 5 &      farsecsq\_MP &    11 &  0 & \quart{11}{0}{11}{100} \\             
% 6 &      train\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\                   
% 6 &      train\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\                  
% 6 &      train\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\                   
% 6 &      farsec\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\                  
% 6 &      clnifarsec\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\              
% 6 &      clni\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\                    
% 6 &      clni\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\                     
% 6 &      clni\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\                    
% 6 &      train\_LR &    0 &  0 & \quart{0}{0}{0}{100} \\                   
% 6 &      farsectwo\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\               
% 6 &      farsec\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\                  
% 6 &      farsec\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\                  
% 6 &      clnifarsec\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\              
% 6 &      clnifarsectwo\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\           
% 6 &      farsec\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\                 
% 6 &      clnifarsec\_KNN &    0 &  0 & \quart{0}{0}{0}{100} \\             
% 6 &      clnifarsec\_RF &    0 &  0 & \quart{0}{0}{0}{100} \\              
% 6 &      clni\_MP &    0 &  0 & \quart{0}{0}{0}{100} \\                    
% 6 &      farsectwo\_KNN &    6 &  0 & \quart{6}{0}{6}{100} \\              
% 6 &      clnifarsectwo\_KNN &    6 &  0 & \quart{6}{0}{6}{100} \\          
% 6 &      farsectwo\_LR &    6 &  0 & \quart{6}{0}{6}{100} \\               
% 6 &      farsectwo\_RF &    6 &  0 & \quart{6}{0}{6}{100} \\               
% 6 &      clnifarsectwo\_LR &    6 &  0 & \quart{6}{0}{6}{100} \\           
% 6 &      clnifarsecsq\_KNN &    6 &  0 & \quart{6}{0}{6}{100} \\           
% 6 &      farsecsq\_KNN &    6 &  0 & \quart{6}{0}{6}{100} \\               
% 6 &      clnifarsectwo\_RF &    6 &  6 & \quart{0}{6}{6}{100} \\           
%     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %   1 & clnifarsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   1 &     farsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   2 &    farsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 & clnifarsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &       farsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &   clnifarsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   3 &         clni &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %   3 &        train &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   1 & farsectwo\_RF\_DE &    0.77  &  0.0 & \quart{79}{0}{79}{109} \\
% %   2 &    farsectwo &    0.56  &  0.42 & \quart{0}{53}{53}{109} \\
% %   2 & clnifarsectwo &    0.56  &  0.0 & \quart{53}{0}{53}{109} \\
% %   3 &         clni &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 & clnifarsecsq &    0.14  &  0.14 & \quart{0}{17}{0}{109} \\
% %   3 &        train &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 &     farsecsq &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %   3 &       farsec &    0.28  &  0.0 & \quart{17}{0}{17}{109} \\
% %   3 &   clnifarsec &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %   1 &       farsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\
% %   1 &   clnifarsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\ 
% %   2 &         clni &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &        train &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &     farsecsq &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   3 & clnifarsecsq &    0.11  &  0.0 & \quart{24}{0}{24}{469} \\
% %   4 &    farsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %   4 & clnifarsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %   1 & farsectwo\_RF\_DE &    0.68  &  0.0 & \quart{79}{0}{79}{132} \\
% %   2 & clnifarsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   2 &     farsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   3 &       farsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   3 &   clnifarsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   4 &        train &    0.45  &  0.0 & \quart{42}{0}{42}{132} \\
% %   5 & clnifarsectwo &    0.38  &  0.05 & \quart{22}{9}{31}{132} \\
% %   5 &    farsectwo &    0.43  &  0.05 & \quart{34}{8}{39}{132} \\
% %   6 &         clni &    0.21  &  0.05 & \quart{0}{8}{3}{132} \\



%  %%% ----END HERE---------------------------------
%   \end{tabular}} \end{minipage}}\hspace{12mm}
% \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% % \begin{center}b. TPP results wit FARSEC and CLNI filtering\end{center}

% % \noindent \begin{tabular}{llrrc}
% %   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% %   \nm{Chromium}\\
% %  \rowcolor{gray!20}   1* &      train &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec &    69 &  18 & \quart{69}{18}{76}{100} \\
% %  \rowcolor{gray!20}   1* &      train\_DE &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq\_DE &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo\_DE &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec\_DE &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni\_DE &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq\_DE &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     \\
% %     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %     1 &      train &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo &    178 &  122 & \ofr \\
% %     4 &      clnifarsec &    178 &  122 & \ofr \\
% %     1 &      train\_DE &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq\_DE &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo\_DE &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq\_DE &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo\_DE &    178 &  122 & \ofr \\
% %     4 &      clnifarsec\_DE &    178 &  122 & \ofr \\
% %     \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   \rowcolor{gray!20}   1* &      train &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec &    56 &  33 & \quart{38}{33}{56}{100} \\
% %   \rowcolor{gray!20}   1* &      train\_DE &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq\_DE &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo\_DE &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec\_DE &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni\_DE &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq\_DE &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %     \rowcolor{gray!20}   1* &      train &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq\_DE &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo\_DE &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec\_DE &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni\_DE &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq\_DE &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo\_DE &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec\_DE &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %     \rowcolor{gray!20}   1* &      train &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec &    99 &  444 & \ofr \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq\_DE &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo\_DE &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec\_DE &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni\_DE &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq\_DE &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo\_DE &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec\_DE &    99 &  444 & \ofr \\

% %   %%% ----END HERE----------------------------------
   
   
% %   \end{tabular}
%   }

% \end{minipage}
% }
%  \caption{
% \%  WPP and TPP precision results of using default hyperparameter in scikit-learn and tuning using differential evolutionary (DE) algorithm
%   }
%  \label{fig:jur}
% \end{figure*}



% \begin{figure*}
% \renewcommand{\baselinestretch}{0.65} 
%  \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% \vspace{2.5mm}
% \begin{center}a. The recall results of project Derby with FARSEC and CLNI filtering\end{center}
% \noindent \begin{tabular}{llrrc}
%   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% 1 &      farsecsq\_MP &    95 &  3 & \quart{95}{3}{95}{100} \\
%     1 &      clnifarsecsq\_NB &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_KNN\_DE3 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_MP\_DE3 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_MP\_DE20 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_NB &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_RF\_DE20 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_RF\_DE10 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_RF\_DE20 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsedsq\_MP\_DE10 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_MP\_DE20 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_RF\_DE3 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_RF\_DE3 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_RF\_DE10 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_LR &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_KNN\_DE10 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_MP &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_MP\_DE3 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      farsecsq\_MP\_DE10 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     1 &      clnifarsecsq\_KNN\_DE20 &    100 &  0 & \quart{100}{0}{100}{100} \\
%     2 &      farsectwo\_MP\_DE20 &    81 &  0 & \quart{81}{0}{81}{100} \\
%     2 &      clnifarsectwo\_NB &    81 &  0 & \quart{81}{0}{81}{100} \\
%     2 &      clnifarsectwo\_MP\_DE3 &    81 &  2 & \quart{81}{2}{81}{100} \\
%     2 &      farsectwo\_NB &    81 &  0 & \quart{81}{0}{81}{100} \\
%     2 &      clnifarsectwo\_MP\_DE10 &    81 &  5 & \quart{81}{5}{81}{100} \\
%     2 &      clnifarsectwo\_MP\_DE20 &    81 &  5 & \quart{81}{5}{81}{100} \\
%     2 &      farsectwo\_MP\_DE10 &    86 &  5 & \quart{81}{5}{86}{100} \\
%     3 &      farsecsq\_RF &    62 &  4 & \quart{60}{4}{62}{100} \\
%     3 &      clnifarsecsq\_RF &    67 &  4 & \quart{67}{4}{67}{100} \\
%     3 &      farsectwo\_MP\_DE3 &    69 &  4 & \quart{67}{4}{69}{100} \\
%     3 &      farsecsq\_LR &    71 &  0 & \quart{71}{0}{71}{100} \\
%     4 &      clnifarsecsq\_KNN &    60 &  0 & \quart{60}{0}{60}{100} \\
%     4 &      farsecsq\_KNN\_DE3 &    60 &  0 & \quart{60}{0}{60}{100} \\
%     4 &      clnifarsectwo\_LR &    60 &  0 & \quart{60}{0}{60}{100} \\
%     4 &      farsecsq\_KNN\_DE10 &    60 &  0 & \quart{60}{0}{60}{100} \\
%     4 &      farsecsq\_KNN\_DE20 &    60 &  0 & \quart{60}{0}{60}{100} \\
%     4 &      farsecsq\_KNN &    60 &  0 & \quart{60}{0}{60}{100} \\
%     4 &      farsectwo\_LR &    60 &  0 & \quart{60}{0}{60}{100} \\
%     5 &      clnifarsectwo\_RF\_DE20 &    56 &  1 & \quart{55}{1}{56}{100} \\
%     6 &      farsectwo\_RF\_DE10 &    52 &  0 & \quart{52}{0}{52}{100} \\
%     6 &      farsectwo\_RF\_DE20 &    55 &  3 & \quart{52}{3}{55}{100} \\
%     6 &      clnifarsectwo\_RF\_DE10 &    55 &  0 & \quart{55}{0}{55}{100} \\
%     7 &      farsectwo\_RF\_DE3 &    50 &  2 & \quart{50}{2}{50}{100} \\
%     7 &      clnifarsectwo\_RF\_DE3 &    50 &  0 & \quart{50}{0}{50}{100} \\
%     8 &      clnifarsec\_NB &    48 &  0 & \quart{48}{0}{48}{100} \\
%     8 &      farsec\_NB &    48 &  0 & \quart{48}{0}{48}{100} \\
%     9 &      train\_NB &    45 &  0 & \quart{45}{0}{45}{100} \\
%     9 &      clni\_NB &    45 &  0 & \quart{45}{0}{45}{100} \\
%     10 &      clnifarsec\_MP\_DE20 &    38 &  2 & \quart{38}{2}{38}{100} \\
%     10 &      farsec\_MP\_DE20 &    40 &  7 & \quart{38}{7}{40}{100} \\
%     10 &      farsectwo\_MP &    40 &  3 & \quart{40}{3}{40}{100} \\
%     10 &      clnifarsectwo\_MP &    43 &  5 & \quart{43}{5}{43}{100} \\
%     10 &      clnifarsectwo\_RF &    43 &  7 & \quart{36}{7}{43}{100} \\
%     11 &      clni\_MP\_DE20 &    36 &  0 & \quart{36}{0}{36}{100} \\
%     11 &      clnifarsec\_RF\_DE20 &    36 &  0 & \quart{36}{0}{36}{100} \\
%     11 &      farsectwo\_RF &    36 &  4 & \quart{36}{4}{36}{100} \\
%     11 &      clnifarsec\_MP\_DE10 &    36 &  7 & \quart{31}{7}{36}{100} \\
%     12 &      clni\_RF\_DE10 &    33 &  0 & \quart{33}{0}{33}{100} \\
%     12 &      farsec\_RF\_DE10 &    33 &  0 & \quart{33}{0}{33}{100} \\
%     12 &      train\_MP\_DE10 &    33 &  2 & \quart{31}{2}{33}{100} \\
%     12 &      train\_MP\_DE20 &    33 &  2 & \quart{31}{2}{33}{100} \\
%     12 &      farsec\_MP\_DE10 &    33 &  2 & \quart{31}{2}{33}{100} \\
%     12 &      clni\_RF\_DE20 &    33 &  0 & \quart{33}{0}{33}{100} \\
%     12 &      clnifarsec\_RF\_DE10 &    33 &  3 & \quart{33}{3}{33}{100} \\
%     12 &      clnifarsec\_RF\_DE3 &    33 &  0 & \quart{33}{0}{33}{100} \\
%     12 &      farsec\_RF\_DE20 &    33 &  3 & \quart{33}{3}{33}{100} \\
%     13 &      clni\_MP\_DE10 &    31 &  7 & \quart{28}{7}{31}{100} \\
%     13 &      clnifarsec\_MP &    31 &  2 & \quart{28}{2}{31}{100} \\
%     13 &      clnifarsec\_MP\_DE3 &    31 &  2 & \quart{28}{2}{31}{100} \\
%     13 &      train\_RF\_DE20 &    31 &  0 & \quart{31}{0}{31}{100} \\
%     13 &      clnifarsec\_LR &    31 &  0 & \quart{31}{0}{31}{100} \\
%     13 &      train\_RF\_DE10 &    31 &  2 & \quart{28}{2}{31}{100} \\
%     13 &      clni\_RF\_DE3 &    31 &  0 & \quart{31}{0}{31}{100} \\
%     13 &      farsec\_RF\_DE3 &    31 &  2 & \quart{31}{2}{31}{100} \\
%     14 &      farsec\_MP\_DE3 &    28 &  5 & \quart{26}{5}{28}{100} \\
%     14 &      train\_RF\_DE3 &    28 &  2 & \quart{26}{2}{28}{100} \\
%     14 &      farsec\_LR &    28 &  0 & \quart{28}{0}{28}{100} \\
%     14 &      clni\_MP\_DE3 &    28 &  2 & \quart{26}{2}{28}{100} \\
%     15 &      clnifarsectwo\_KNN\_DE20 &    26 &  0 & \quart{26}{0}{26}{100} \\
%     15 &      clnifarsectwo\_KNN\_DE3 &    26 &  0 & \quart{26}{0}{26}{100} \\
%     15 &      clnifarsectwo\_KNN &    26 &  0 & \quart{26}{0}{26}{100} \\
%     15 &      clnifarsectwo\_KNN\_DE10 &    26 &  0 & \quart{26}{0}{26}{100} \\
%     16 &      clni\_LR &    24 &  0 & \quart{24}{0}{24}{100} \\
%     16 &      train\_MP\_DE3 &    24 &  2 & \quart{24}{2}{24}{100} \\
%     16 &      clnifarsec\_RF &    24 &  5 & \quart{21}{5}{24}{100} \\
%     16 &      train\_LR &    24 &  0 & \quart{24}{0}{24}{100} \\
%     17 &      train\_MP &    21 &  2 & \quart{19}{2}{21}{100} \\
%     17 &      farsectwo\_KNN &    21 &  0 & \quart{21}{0}{21}{100} \\
%     17 &      clni\_MP &    21 &  4 & \quart{17}{4}{21}{100} \\
%     17 &      farsectwo\_KNN\_DE3 &    21 &  0 & \quart{21}{0}{21}{100} \\
%     17 &      clni\_RF &    21 &  0 & \quart{21}{0}{21}{100} \\
%     17 &      farsectwo\_KNN\_DE10 &    21 &  0 & \quart{21}{0}{21}{100} \\
%     17 &      farsectwo\_KNN\_DE20 &    21 &  0 & \quart{21}{0}{21}{100} \\
%     17 &      farsec\_MP &    21 &  5 & \quart{19}{5}{21}{100} \\
%     18 &      clnifarsec\_KNN\_DE20 &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clni\_KNN &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      farsec\_RF &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clni\_KNN\_DE10 &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      train\_RF &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clni\_KNN\_DE3 &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clnifarsec\_KNN\_DE3 &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clni\_KNN\_DE20 &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clnifarsec\_KNN\_DE10 &    19 &  0 & \quart{19}{0}{19}{100} \\
%     18 &      clnifarsec\_KNN &    19 &  0 & \quart{19}{0}{19}{100} \\
%     19 &      train\_KNN &    12 &  2 & \quart{12}{2}{12}{100} \\
%     19 &      train\_KNN\_DE3 &    12 &  2 & \quart{12}{2}{12}{100} \\
%     19 &      farsec\_KNN\_DE20 &    14 &  2 & \quart{12}{2}{14}{100} \\
%     19 &      farsec\_KNN &    14 &  2 & \quart{12}{2}{14}{100} \\
%     19 &      farsec\_KNN\_DE3 &    14 &  2 & \quart{12}{2}{14}{100} \\
%     19 &      train\_KNN\_DE20 &    14 &  2 & \quart{12}{2}{14}{100} \\
%     19 &      train\_KNN\_DE10 &    14 &  2 & \quart{12}{2}{14}{100} \\
%     19 &      farsec\_KNN\_DE10 &    14 &  0 & \quart{14}{0}{14}{100} \\
%     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %   1 & clnifarsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   1 &     farsecsq &    0.83  &  0.0 & \quart{79}{0}{79}{96} \\
% %   2 &    farsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 & clnifarsectwo &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &       farsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   2 &   clnifarsec &    0.67  &  0.0 & \quart{64}{0}{64}{96} \\
% %   3 &         clni &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %   3 &        train &    0.0  &  0.0 & \quart{0}{0}{0}{96} \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   1 & farsectwo\_RF\_DE &    0.77  &  0.0 & \quart{79}{0}{79}{109} \\
% %   2 &    farsectwo &    0.56  &  0.42 & \quart{0}{53}{53}{109} \\
% %   2 & clnifarsectwo &    0.56  &  0.0 & \quart{53}{0}{53}{109} \\
% %   3 &         clni &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 & clnifarsecsq &    0.14  &  0.14 & \quart{0}{17}{0}{109} \\
% %   3 &        train &    0.14  &  0.0 & \quart{0}{0}{0}{109} \\
% %   3 &     farsecsq &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %   3 &       farsec &    0.28  &  0.0 & \quart{17}{0}{17}{109} \\
% %   3 &   clnifarsec &    0.28  &  0.14 & \quart{0}{17}{17}{109} \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %   1 &       farsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\
% %   1 &   clnifarsec &    0.22  &  0.0 & \quart{79}{0}{79}{469} \\ 
% %   2 &         clni &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &        train &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   2 &     farsecsq &    0.17  &  0.0 & \quart{54}{0}{54}{469} \\
% %   3 & clnifarsecsq &    0.11  &  0.0 & \quart{24}{0}{24}{469} \\
% %   4 &    farsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %   4 & clnifarsectwo &    0.06  &  0.0 & \quart{0}{0}{0}{469} \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %   1 & farsectwo\_RF\_DE &    0.68  &  0.0 & \quart{79}{0}{79}{132} \\
% %   2 & clnifarsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   2 &     farsecsq &    0.6  &  0.0 & \quart{66}{0}{66}{132} \\
% %   3 &       farsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   3 &   clnifarsec &    0.48  &  0.0 & \quart{47}{0}{47}{132} \\
% %   4 &        train &    0.45  &  0.0 & \quart{42}{0}{42}{132} \\
% %   5 & clnifarsectwo &    0.38  &  0.05 & \quart{22}{9}{31}{132} \\
% %   5 &    farsectwo &    0.43  &  0.05 & \quart{34}{8}{39}{132} \\
% %   6 &         clni &    0.21  &  0.05 & \quart{0}{8}{3}{132} \\



%  %%% ----END HERE---------------------------------
%   \end{tabular}} \end{minipage}}\hspace{12mm}
% \resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
% {\small
% % \begin{center}b. TPP results wit FARSEC and CLNI filtering\end{center}

% % \noindent \begin{tabular}{llrrc}
% %   {\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\\hline
  
% %   \nm{Chromium}\\
% %  \rowcolor{gray!20}   1* &      train &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec &    69 &  18 & \quart{69}{18}{76}{100} \\
% %  \rowcolor{gray!20}   1* &      train\_DE &    8 &  1 & \quart{7}{1}{8}{100} \\
% %  \rowcolor{gray!20}   1* &      farsecsq\_DE &    9 &  2 & \quart{8}{2}{9}{100} \\ 
% %     2 &     farsectwo\_DE &    15 &  2 & \quart{14}{2}{15}{100} \\
% %     3 &     farsec\_DE &    33 &  12 & \quart{26}{12}{33}{100} \\
% %     4 &     clni\_DE &    40 &  10 & \quart{37}{10}{40}{100} \\ 
% %     5 &     clnifarsecsq\_DE &    54 &  10 & \quart{47}{10}{54}{100} \\ 
% %     6 &     clnifarsectwo\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     6 &     clnifarsec\_DE &    69 &  18 & \quart{69}{18}{76}{100} \\
% %     \\
% %     \\
% %     \hline
% %   %%% generating from latex_plotting.py::plot_mre_for_all
% % \nm{Wicket}\\
% %     1 &      train &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo &    178 &  122 & \ofr \\
% %     4 &      clnifarsec &    178 &  122 & \ofr \\
% %     1 &      train\_DE &    48 &  29 & \quart{36}{29}{48}{100} \\
% %     1 &      farsecsq\_DE &    48 &  20 & \quart{40}{20}{48}{100} \\
% %     1 &      farsectwo\_DE &    51 &  30 & \quart{36}{30}{51}{100} \\
% %     2 &      farsec\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clni\_DE &    56 &  23 & \quart{48}{23}{56}{100} \\
% %     2 &      clnifarsecsq\_DE &    59 &  21 & \quart{48}{21}{59}{100} \\
% %     4 &      clnifarsectwo\_DE &    178 &  122 & \ofr \\
% %     4 &      clnifarsec\_DE &    178 &  122 & \ofr \\
% %     \\
% %     \\
% %     \hline
% % \nm{Ambari}\\
% %   \rowcolor{gray!20}   1* &      train &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec &    56 &  33 & \quart{38}{33}{56}{100} \\
% %   \rowcolor{gray!20}   1* &      train\_DE &    39 &  19 & \quart{31}{19}{39}{100} \\
% %   \rowcolor{gray!20}   1* &      farsecsq\_DE &    41 &  19 & \quart{31}{19}{41}{100} \\
% %   \rowcolor{gray!20}   1* &      farsectwo\_DE &    43 &  18 & \quart{33}{18}{43}{100} \\
% %     2 &      farsec\_DE &    45 &  18 & \quart{37}{18}{46}{100} \\
% %     2 &      clni\_DE &    46 &  18 & \quart{37}{18}{46}{100} \\
% %     3 &      clnifarsecsq\_DE &    51 &  17 & \quart{46}{17}{51}{100} \\
% %     3 &      clnifarsectwo\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     3 &      clnifarsec\_DE &    56 &  33 & \quart{38}{33}{56}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Camel}\\
% %     \rowcolor{gray!20}   1* &      train &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    14 &  12 & \quart{8}{12}{14}{100} \\
% %     2 &      farsecsq\_DE &    23 &  18 & \quart{15}{18}{23}{100} \\
% %     2 &      tarsectwo\_DE &    24 &  16 & \quart{16}{16}{24}{100} \\
% %     2 &      farsec\_DE &    30 &  11 & \quart{24}{11}{30}{100} \\
% %     2 &      clni\_DE &    32 &  16 & \quart{25}{16}{32}{100} \\
% %     3 &      clnifarsecsq\_DE &    43 &  26 & \quart{34}{26}{43}{100} \\
% %     4 &      clnifarsectwo\_DE &    53 &  32 & \quart{49}{32}{53}{100} \\
% %     6 &      clnifarsec\_DE &    87 &  72 & \quart{49}{57}{87}{100} \\
% %     \\
% %     \\
% %     \hline
% % \nm{Derby}\\
% %     \rowcolor{gray!20}   1* &      train &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec &    99 &  444 & \ofr \\
% %     \rowcolor{gray!20}   1* &      train\_DE &    36 &  21 & \quart{31}{21}{33}{100} \\
% %     2 &      farsecsq\_DE &    46 &  15 & \quart{31}{15}{43}{100} \\
% %     2 &      farsectwo\_DE &    54 &  22 & \quart{41}{22}{54}{100} \\
% %     2 &      farsec\_DE &    55 &  38 & \quart{32}{38}{55}{100} \\
% %     3 &      clni\_DE &    61 &  21 & \quart{49}{21}{61}{100} \\
% %     3 &      clnifarsecsq\_DE &    61 &  20 & \quart{52}{20}{61}{100} \\
% %     3 &      clnifarsectwo\_DE &    62 &  15 & \quart{54}{15}{62}{100} \\
% %     4 &      clnifarsec\_DE &    99 &  444 & \ofr \\

% %   %%% ----END HERE----------------------------------
   
   
% %   \end{tabular}
%   }

% \end{minipage}
% }
%  \caption{
% \%  WPP and TPP precision results of using default hyperparameter in scikit-learn and tuning using differential evolutionary (DE) algorithm
%   }
%  \label{fig:jur}
% \end{figure*}

==> section/introduction.tex <==
\section{Introduction}
\begin{itemize}
    \item \textbf{RQ1: Which tool is better for retrieving SATD?}
    \item \textbf{RQ2: Given a new Dataset, can we say how much SATD it contains?}
    \item \textbf{RQ3: How early can we estimate SATD?}
    \item \textbf{RQ4: Can SATD be confirmed in a cost-effective manner?}
    \item \textbf{RQ5: How much background knowledge do we need?}
\end{itemize}


==> section/results.tex <==
\section{Results}
\label{ch results}


